A Declarative Metamorphic Testing Framework for Autonomous Driving

Autonomous driving has gained much attention from both industry and academia. Currently, Deep Neural Networks (DNNs) are widely used for perception and control in autonomous driving. However, several fatal accidents caused by autonomous vehicles have raised serious safety concerns about autonomous driving models. Some recent studies have successfully used the metamorphic testing technique to detect thousands of potential issues in some popularly used autonomous driving models. However, prior study is limited to a small set of metamorphic relations, which do not reflect rich, real-world traffic scenarios and are also not customizable. This paper presents a novel declarative rule-based metamorphic testing framework called RMT. RMT provides a rule template with natural language syntax, allowing users to flexibly specify an enriched set of testing scenarios based on real-world traffic rules and domain knowledge. RMT automatically parses human-written rules to metamorphic relations using an NLP-based rule parser referring to an ontology list and generates test cases with a variety of image transformation engines. We evaluated RMT on three autonomous driving models. With an enriched set of metamorphic relations, RMT detected a significant number of abnormal model predictions that were not detected by prior work. Through a large-scale human study on Amazon Mechanical Turk, we further confirmed the authenticity of test cases generated by RMT and the validity of detected abnormal model predictions.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)

==> background.tex <==
\section{Background}
\label{sec:background}
%\vspace{-2pt}
\subsection{Metamorphic testing}
%\vspace{-2pt}
Metamorphic testing (MT) was proposed by Chen et al.~\cite{chen1998metamorphic} to address the oracle problem, because without the test oracle (a correct expected system output), most testing techniques cannot work. Given source test cases with corresponding outputs, MT uses metamorphic relations (MRs) to generate follow-up test cases (new test cases) with modified outputs. MRs are the pre-defined relationships between the results of source test cases and follow-up test cases. When test results violate MRs, software might have robustness problems. Suppose a program \(f\) implemented the SINE function, and we do not have correct output of corresponding test input to verify the correctness of the software. However, we could define an MR, \(f(x) = f(x + 2\pi)\). Then we could generate follow-up test case \(x + 2\pi\) and verify the correctness of the program by checking the output consistency of original outcome \(f(x)\) and the follow-up test outcome \(f(x +2\pi)\)~\cite{chen2016metric}. 

Now MT is widely applied in many domains like Web~\cite{chan2007metamorphic}, middleware~\cite{chan2006integration}, healthcare~\cite{murphy2011effective}, and machine learning~\cite{xie2011testing}, where it is extremely difficult and time-consuming to declare test oracle functions. For machine learning, in 2008, Murphy et al.~\cite{murphy2008properties} proposed six MRs to transform input data including additive, multiplicative, permutative, invertive, inclusive, and exclusive. They analyzed availability of those MRs in supervised and unsupervised machine learning algorithms. Based on the work, in 2009, Xie et al.~\cite{xie2011testing} implemented MRs to test specific supervised machine learning models like K-Nearest Neighbour (KNN) and Naive Bayes classifier. %Recently, Zhang et al. proposed DeepRoad~\cite{zhang2018deeproad} to generate new test cases based on the metamorphic relation that the steering angle of an autonomous vehicle should not change when the driving scenes are synthesized with different weather conditions. In this way metamorphic testing could generate more test cases to cover extreme test scenarios so as to verify the robustness of autonomous driving models.
%\vspace{-8pt}
\subsection{Autonomous driving model}
%\vspace{-2pt}
Figure~\ref{driving-model-arch} shows the basic structure of an autonomous driving model. Given input data from sensors (e.g. LiDARs and cameras), control of vehicle like steering angel and speed is outputted by a deep neural network model. CNN, with its excellent performance on precision, space and time consumption, becomes a mainstream neural network architecture used for autonomous driving models. 
In 1989, the fully connected neural network was proposed to control a vehicle~\cite{pomerleau1989alvinn}. In 2003, DAVE~\cite{lecun2004dave} was proposed as an autonomous driving model that successfully controlled a vehicle drive around an alley. Then Nvidia proposed DAVE-2, which is a CNN-based autonomous driving model to predict steering angle~\cite{bojarski2016end}. They demonstrated that DAVE-2 can automatically {\color{blue}to} drive a vehicle without human intervention in 90\% of the time in a simulation test while performing autonomous steering in 98\% of time in an on-road test. A self-driving startup \textit{comma.ai} presented a CNN model to predict steering angle based on driving videos~\cite{santana2016learning}. In Udacity challenge~\cite{Udacity}, the top-ranked model, Komanda, which is based on 3D-CNN and long short-term memory (LSTM), could simultaneously predict a steering angle, torque, and speed.
%Figure~\ref{driving-model-arch} shows the basic structure of an autonomous driving model. Given input data from sensors (e.g., LiDARs and cameras), a deep neural network outputs the control of the vehicle like steering angle and speed. Due to excellent performance, requiring less neurons and consuming less resource, CNN is the mainstream neural network architecture used for autonomous driving models. In 1989, the fully connected neural network was proposed to control a vehicle~\cite{pomerleau1989alvinn}. In 2003, DAVE~\cite{lecun2004dave} was proposed as an autonomous driving model that successfully controlled a vehicle drive around an alley. Then Nvidia proposed DAVE-2, which is a CNN-based autonomous driving model to predict steering angle~\cite{bojarski2016end}. They demonstrate that DAVE-2 can automatically drive a vehicle without human intervention in 90\% of the time in a simulation test while performing autonomous steering in 98\% of time in an on-road test.~\textit{comma.ai} presents a CNN model to predict steering angle based on driving video~\cite{santana2016learning}. In Udacity challenge~\cite{Udacity}, the rank 1 model called Komanda based on 3D CNN and Long short-term memory (LSTM) could simultaneously predict steering angle, torque and speed.
We choose three well-recognized driving models including one Udacity challenge top ranked model. These models predict driving speed given a driving scene image as input. To test such regression models, it is not straightforward to write expressive MRs directly. However it is much easier to translate intuitive traffic rules to corresponding MRs. %define such MRs based on traffic rules.

%\vspace{-8pt}
\subsection{Image generation via GAN}
%\vspace{-2pt}
Generative Adversarial Network (GAN) proposed by Goodfellow et al.~\cite{goodfellow2014generative} has been proven effective on image generation and modification tasks. GAN is designed with a generator-discriminator architecture, which aims to optimize generation network parameters through adversarial training. The generating part (generator) of GAN network normally accepts a noise or a mask as input and generates an image through fully connected or convolution layers, while the discriminating part (discriminator) of a GAN network is trained to discriminate between real images and images generated by the generator. In our work, we use GAN to generate metamorphic test set images for some traffic rules to increase our capability to apply meaningful input image transformation. %some corresponding rules. 

%The loss function of GAN is shown as below:

%\begin{equation}
%\label{GAN}
 %   \mathcal{L}_{GAN} = \mathbb{E}_x log(\mathcal{D}(x) + \mathbb{E}_x log(1 - \mathcal{D}(\mathcal{G}(x)))
%\end{equation}


%After GAN was introduced, researches have been taken place to improve image generation performance based on GAN structure,several effective architectures have been proposed. DCGAN\cite{radford2015unsupervised} is a popular adaptation of GAN utilizing CNN structure for generating natural images. CycleGAN \cite{zhu2017unpaired} introduced a loop architecture modified from the original GAN, which provide a general solution for GAN models training on unpaired image data. CycleGAN makes image to image transformation simpler, especially for tasks like object transfiguration, and season or style transfer etc.
%GAN has also been proven to be used for data augmentation. Antoniou et al.\cite{antoniou2017data} proposed a GAN-based data augmentation model and showed how it outperforms other popular data augmentation models. Study performed by Mariani el al.\cite{mariani2018bagan} also showed how various of GAN based data augmentation improve final classification performance of an image classification model.















 

==> discussion.tex <==
%This section file is obsolete 
%\section{Discussion (Lou)}
%\label{sec:discussion}

%Experiment Condition





==> method_backup.tex <==
\section{The RMT Framework}
\label{sec:methodology}





%\subsection{Overview}
\begin{figure*}[ht]
\centering
\includegraphics[width = 1\textwidth]{images/RMT-TSE.drawio.pdf}
\vspace{-20pt}
\caption{Overview of {\tool}}
\vspace{-6pt}
\label{fig:framework-workflow}
\end{figure*}

{\tool} allows users to interactively and flexibly define custom metamorphic driving scenarios for testing autonomous driving models. Figure \ref{fig:framework-workflow} shows the architecture of {\tool}. It consists of three components: (1) an NLP-based semantic parser that induces metamorphic relations (MRs) from human-written test scenarios, (2) a test generator that generates new road images based on the induced MR, and (3) an anomaly detector that detects MR violations. 

{\color{blue}
First, a user describes a testing rule following the IFTTT paradigm in natural language (Section~\ref{sec:ontology}). The testing rule specifies how to change a driving scenario as well as the expected driving behavior change. Then an NLP-based semantic parser leverages a driving scenario ontology to match and extract key information in the testing rule (Section~\ref{sec:parser}). Then, an MR is established based on the extracted information. Based on this MR, the test generator generates new road images by editing or translating an original image (Section~\ref{sec:MT generator}).
}
% First, a user describes a test scenario in natural language based on the rule template introduced in Section~\ref{sec:template}. Given a rule, the semantic parser will automatically parse it to an metamorphic relation. The transformation operation and parameters recognized from a human-written rule will be fed into the metamorphic test generator for to generate new test cases (i.e., road images). 
% The metamorphic test generator contains various image transformation engines. Each transformation engine can manipulate an original road image and then generate a new metamorphic image. 
% For each MR, the test generator can select the corresponding transformation engine based on a provided configuration file as discussed in
% Section~\ref{sec:configration}. 
% The chosen transformation engine
% will then use the original test image set to
% generate a set of metamorphic images.  
% Note that a transformation may not be applicable to all road images in the original test set. Such cases are filtered out by built-in filters implemented in transformation engines. 
For each pair of the original and the newly generated images, the anomaly detector checks whether the model predictions satisfy the MR. If an MR is violated, an abnormal prediction is detected, indicating a violation of the human-written testing rule. 


% In this paper, we proposed seven traffic rules to demonstrate the expressiveness of {\tool}. Rules 1, 2, and 7 are directly derived from traffic rules from official driver handbooks in three different countries, as shown in Table~\ref{tab:handbook}. These rules check whether a driving model can handle potential hazards (e.g., a pedestrian may cross the road), recognize traffic signs, and recognize different driving scenes (e.g., daytime vs.~nighttime). Rules 3-6 are custom rules. Rule 3 is a customized from Rule 1 with a specific deceleration threshold, which can be set flexibily based on user expectation. Rule 4 extends the traffic rule of NSW in Table~\ref{tab:handbook} to express a more complicated scenario---if the ego-vehicle is getting closer to a pedestrian, it should decelerate more. Rules 5 and 6 are not derived from traffic rules, but they demonstrate how users can specify interesting driving scenes by adding, removing, or replacing objects in a road image. The next section describes  the rule template used to prescribe these rules.

\subsection{Testing Rule Specification}
\label{sec:ontology}

{\color{blue} 
{\tool} accepts testing rules described in natural language based on the IFTTT (If-This-Then-That) paradigm. The IFTTT rule syntax contains one or more {\em if-then} statements. In the {\em if} clause, a user describes how to change a driving scenario. In the {\em then} clause, the user describes the expected driving behavior change caused by the scenario change. %Such an IFTTT description defines an MR that the change of a scenario causes the change of model predictions.
For example, we can specify a testing rule {\em  ``If a pedestrian appears on the roadside, then the ego-vehicle should slow down at least 30\%''}. The {\em if} clause specifies that a driving scenario can be changed by adding a pedestrian on the roadside. The {\em then} clause specifies the expected behavior change, which is the speed of the ego-vehicle should decrease at least 30\%. 

% For the "If" statement, we add a pedestrian entity with the position property on the roadside into the current scenario. For the ``Then" statement, it provides key information {\em target action}, {\em expected change} and {\em change parameters} that describe to what extent the speed of ego-vehicle should decrease. We could also use more ``If...,then'' pairs to describe more scenario change and expected change of driving behaviors. For example, if we add the description ``If the pedestrian becomes closer to the ego-vehicle, then the ego-vehicle should decelerate more.'' following the previous description, we actually change the scenario we created in the first ``If...,then'' pair.

% When a testing rule is created, {\tool} uses a NLP-based semantic parser to extract necessary information such as the class name, properties, and the relation of the ontology entity for scenario generation and metamorphic relation generation. 
}


\subsection{NLP-based Semantic Rule Parsing}
\label{sec:parser}

\begin{comment}
\subsubsection{Rule template}
\label{sec:template}

% \begin{algorithm}
% \caption{Rule template}
% \label{alg:template}

% If:  [\textit{Object}] [\textit{Transformation}] [\textit{Transformation parameter}] \\
% Then: the [\textit{Target action}] of ego-vehicle should [\textit{Expected change}] \textlangle\textit{Change parameter}\textrangle\\
% \textlangle \\
% If: [\textit{Object}] [\textit{Transformation}] [\textit{Transformation parameter}] \\
% Then: the [\textit{Target action}] of ego-vehicle should [\textit{Expected change}] \textlangle\textit{Change parameter}\textrangle\\
% ...\textrangle


% \end{algorithm}

% \begin{algorithm}
% \caption{Rule template}
% \label{alg:template}
% {\color{blue}
% If:  The description of the modified ontology ([\textit{Ontology entity}] [\textit{Ontology property}] [\textit{Ontology transformation}]) \\
% Then: the [\textit{Target action}] of ego-vehicle should [\textit{Expected change}] \textlangle\textit{Change parameter}\textrangle\\
% \textlangle \\
% If: The description of the modified ontology ([\textit{Ontology entity}] [\textit{Ontology property}] [\textit{Ontology transformation}] \textlangle\textit{Ontology relation}\textrangle) \\
% Then: the [\textit{Target action}] of ego-vehicle should [\textit{Expected change}] \textlangle\textit{Change parameter}\textrangle\\
% ...\textrangle
% }

% \end{algorithm}


{\color{blue}We create a rule template based on the IFTTT (If-This-Then-That) programming paradigm as shown in the Rule template Box. In the ``If" statement, a user can describe how to change the current scenario. In the ``Then" statement, the user needs to describe the corresponding change of model predictions caused by the scenario change. Such an IFTTT description defines an MR that the change of a scenario cause the change of model predictions. A rule can contain one or more IFTTT description.} 
% We create a rule template based on ``If...Then" pairs as shown in the Rule template Box.
The first ``If...Then" pair creates a basic testing scenario, which describes how to change the current scenario to a new scenario and defines the underlying MR between the model prediction on the original and transformed images.
In the ``If" statement, we define three rule components including \textbf{Object}, \textbf{Transformation}, and \textbf{Transformation parameters}. Transformation specifies how to change the current scenario. Object specifies the object in the scenario which needs to be transformed.
%to apply the transformation. 
Transformation parameters specify necessary parameters for the transformation. In the ``Then" statement, two components \textbf{Target action} and \textbf{Expected change} are created. Target action defines what behavior of ego-vehicle we want to test.
%we focus on. 
Expected change describes the expected model prediction changes between the %original
source test case and the follow-up test case (whether the underlying MR holds). Also, an optional \textbf{Change parameter} can be used to describe additional information related to the expected changes. For example, proposed Rule 1 has one ``If...Then" pair. The values of rule components Object, Transformation, Transformation parameter, Target action, and Expected change are ``pedestrian'', ``Add'', ``Roadside'', ``speed'', and ``decrease'' respectively.

%is possibly used to help describe the expected change more specifically in the ``Then" statement.
In addition, another ``If...Then" pair can be added in our rules to create a more complicated testing scenario. In such case, we can use the first ``If...Then" pair to generate follow-up test cases (first-order metamorphic test cases) and check whether the underlying MR holds. Based on new follow-up test cases, we can generate more complex follow-up test cases (second-order metamorphic test cases) using the second ``If...Then" pair and compare whether the newly specified MR holds between the first-order and the second-order metamorphic test cases. For example, the proposed Rule 4 has two ``If...Then" pairs. in the first ``If" statement, we create a scenario by adding a pedestrian at the roadside, while in the  second ``If'' statement, we specify the previously added pedestrian is closer to the ego-vehicle by another transformation parameter {\textit closer}. The second ``Then" statement creates an MR between predictions on two transformed driving scenes. In this paper, we only use second-order metamorphic test cases once in Rule 4 (one nested ``If...Then'' pair), but our rule template does not restrict exploring higher-order metamorphic test cases (more than one nested ``If...Then" pairs). Moreover, in ``If'' statement, we restrict the description using passive tone to automate the rule processing by our NLP-based parser in Section~\ref{sec:parser}. 

Table~\ref{tab:template_p2} shows the set of transformations, objects, and parameters supported by our current prototype. Our prototype supports
four transformations including \textit{Add}, \textit{Remove}, \textit{Update} and \textit{Replace}. 
%are defined in the rule template.
Each transformation can be applied on specific objects in the driving scenes, some of which may require specific transformation parameters. The \textit{Add} transformation 
can be used to add pedestrians and slow speed signs. It also requires a transformation parameter to specify the location of added objects, either at \textit{Roadside} or \textit{Closer} to the ego-vehicle. Similarly, for the \textit{Update} transformation, we allow updating the \textit{Time} of a driving scene from \textit{Day} to \textit{Night}. For the \textit{Replace} transformation, we allow replacing the \textit{Buildings} in a driving scene to \textit{Trees}.
The \textit{Remove} transformation can be used to remove \textit{Lane Lines} in a driving scene. The implementation details of these transformations are described in Section~\ref{sec:MT generator}.

\begin{table*}[!t]
\centering
\caption{Transformations, objects, and parameter values supported by our current prototype}
\label{tab:template_p2}
\begin{tabular}{l|l|l|l|l}
\hline
\textbf{Transformation}      & \textbf{Add}                                                          & \textbf{Remove} & \textbf{Update}     & \textbf{Replace}     \\ \hline
\textbf{Object}              & \begin{tabular}[c]{@{}l@{}}Pedestrian;\\ Slow speed sign\end{tabular} & Lane lines      & Time                & Buildings            \\ \hline
\textbf{Transform parameter} & Location: Roadside; Closer                                                   &        -         & Target style: Night & Target object: Trees \\ \hline
\textbf{Target action}       & \multicolumn{4}{l}{Speed; Steering angle}                                                                                           \\ \hline
\textbf{Expected change}     & \multicolumn{4}{l}{Increase; Decrease; Keep the same}                                                                                   \\ \hline
\textbf{Change parameter}    & \multicolumn{4}{l}{At least; More}                                                                                                  \\ \hline
\end{tabular}
\vspace{-15pt}
\end{table*}


Currently, our prototype supports two target actions to be monitored for MR violations, one is \textit{Speed} and the other is \textit{Steering angle}. They are set based on the prediction types from the driving models. Expected change is set to \textit{Increase}, \textit{Decrease}, and \textit{Keep the same} for now to compare model predictions on the source and transformed images. Sometimes we need to specify the range of changes, so that we set \textit{At least} and \textit{More} for Change parameter. For example, \textit{At least} is used in Rule 4 to specify the speed shall decrease at least 30\% and \textit{more} is used in Rule 5 to specify compared with the model prediction on the first transformed image, the predicted speed on the second transformed image should be smaller.
\end{comment}

% Grammatically dependency analysis a 
% step 1: extract all information from the given testing rule
% step 2: use ontology to match the information and create the ontology entity
% step 3: based on the ontology entity, test generator creates new road images.
% step 4: build MR based on the ontology and 
\subsubsection{Information Extraction}

% extract all dependencies and represent them as predicates: dependency(a, b)
{\color{blue}

\begin{figure}[ht]
\centering
\includegraphics[width = 0.45\textwidth]{images/dependency_parsing.pdf}

\caption{An example of dependency parsing}

\label{fig:dependency}
\end{figure}

Since a testing rule is described in natural language, we propose an NLP-based semantic parser to extract key information from the rule. Given a testing rule, the parser first splits the rule into {\em if} and {\em then} clauses. Then, for each clause, the parser applies POS tagging to identify all nouns, verbs, and adjectives in a sentence. As shown in  Figure~\ref{fig:dependency}, given a sentence, ``{\em a pedestrian appears on the roadside}'', words such as {\em pedestrian, appears, and roadside} are recognized. Then dependency parsing~\cite{yamada2003statistical} is applied to identify the grammar structure between these words. Our semantic parser first parses a sentence to a dependency tree . The root of the tree is the predicate verb, representing by the red node as shown in Figure \ref{fig:dependency}. Then it analyzes other elements such as subjects and objects and identify the grammar dependencies between them. For example, in Figure \ref{fig:dependency}, dependency analysis identifies the root verb {\em appears} and extracts a dependency from {\em appears} to {\em pedestrian} represented by the {\em NSUBJ} tag, which means {\em pedestrian} is the {\em nominal subject} of the verb. Our semantic parser then creates a dependency predicate {\em NSUBJ (pedestrian, appears)} to save the dependency. In addition, sometimes a verb and a noun does not have the direct dependency. The parser extracts the indirect dependency by traversing the dependency tree from the root node verb to the leaf node noun. Then it uses the name of the middle node between the root node and leaf node as the predicate name. For example, in Figure \ref{fig:dependency}, the dependency between {\em appears} and {\em roadside} is represented as dependency predicate {\em ON(roadside, appears)}. If there are adjectives in a sentence, following the same process, dependency predicates between adjectives and nouns are also extracted as {\em amod(noun, adj)}. These extracted dependency predicates are further used to match the ontology in Section \ref{sec:ontology}.

Following the same process, for the {\em then} clause {\em the car should slow down at least 30\%}, we extract dependency predicates {\em {\em NSUBJ(car, slow)}, {\em NPADVMOD(30\%, slow), and {\em ADVMOD(30\%, least)}}. These extracted dependency predicates are used to create an MR in Section \ref{sec:MT generator}}. 

% For the extracted nouns in a sentence, we also applied NER to identify their categories and use the category information to infer more necessary information. For example, for {\em 30 km/h}, NER identifies it as a number of speed. Then we know the testing rule aims to test driving models for speed prediction. 



% POS analysis identifies the part-of-speech of each word in a sentence. NER identifies the category (e.g., person, number, and percentage) of each word or phrase in a sentence. 

% We use spaCy~\cite{spacy} to implement dependency parsing, Part-of-Speech (POS) analysis~\cite{gimpel2010part}, Named Entity Recognition (NER)~\cite{nadeau2007survey}, and word2vec~\cite{mikolov2013efficient}.

% For an {\em if} clause, the subject, the object, and predicate verb are extracted since they are likely to specify the entities to be changed and how to change it. For the previous example ``If a pedestrian appears on the roadside'', {\em pedestrian} and {\em appear} will be extracted. For the change of driving scenario, we currently support three transformations, including {\em add, Remove, and Replace}. The \textit{Add} transformation can be used to add an entity into current scenario. The \textit{Remove} transformation can remove an entity from the driving scenario. For the \textit{Replace} transformation, it could change an entity to another one in the current scenario (e.g., replacing \textit{Buildings} to \textit{Trees}; replacing \textit{Sunny} weather to \textit{Rainy}). We adopt word2vec technology to convert detected description of change (e.g. appear) to a vector and calculate its distance to vectors of three pre-defined transformations. The closest transformation is identified as the correct one in the testing rule.


% Then by using dependency parsing technique, we can identify words or phrases used for modifying the subject, which provide specific information of the changed element. In the example, {\em on the roadside} is extracted and we can know that the pedestrian needs to be added near the road. Similarly, for ``Then'' statement, we can extract the expected change such as {\em slow down} from the predicate verb. The extent of slow down {\em 30km/h} can be extracted via NER. Though the target behavior {\em speed} is not in the description, it can be inferred from the expected change {\em slow down} and the unit {\em km/h}.

% For the "If" statement, the subject should be class name of the ontology defined in the rule. And the predicate verb should describe the relation of the ontology and current scenario, which could be mapped to corresponding transformation. To do this, {\tool} uses word2vec technology to convert the detected relation and predefined four transformations {\em Add, Remove, Update, and Replace} to vectors and calculate the distance between the relation name and transformations. The closest transformation is identified as the correct one corresponding to the relation name. In addition, properties of the ontology should be adjectives or preposition structures to modify the subject. When this words are extracted, NER is used to identify what properties are described by these words. In the previous testing rule example, ``in the front'' could be extracted by POS analysis and then identified as the description of a position based on NER. Similarly, \textit{Target action} and \textit{Expected change} are the subject and predicate verb of the "Then" statement and they can be extracted. For \textit{Change parameter} in the "Then" statement, it could be a phrase containing a preposition and a percentage value to modify predicate verb so it can be identified by combining dependency parsing and NER. 
}


\subsubsection{Match Driving Scenario Ontology}
{\color{blue} 
% Formalize the entire process


When dependency predicates are extracted, {\tool} matches them with a predefined driving scenario ontology. The aim is to identify the element to change and how to change it. Ontology is a methodology to formally summarize categories and create a knowledge base to organize properties and relations in a specific domain. In this work, we propose to use ontology for modeling elements in a driving scenario. Specifically, we define an ontology containing three categories of elements, as shown in Appendix Table~\ref{tab:appendix_ontology}. All ontology elements and their properties are converted to corresponding vectors by word2vec technique~\cite{mikolov2013efficient}. These vectors are further used to match information in dependency predicates. Figure~\ref{fig:ontology} shows a subset of the proposed driving element ontology.

The first category contains properties of a road such as lane lines and surface type. The second category includes objects in a driving scenario such as pedestrians and vehicles. The third category contains elements about the natural environment such as different weather conditions and light conditions. An element can contain specific properties. For example, a car has color, position, and heading properties.

In addition, we define three ways to change an ontology element in a driving scenario, including {\em Add, Remove,} and {\em Replace}. {\em Add} means a new ontology element such as a car can be added in a driving scenario. An existing element such as a traffic sign can be {\em removed} from a driving scenario. Furthermore, an element can be replaced by another element. For example, a white car is replaced with a black car, or the sunny day is replaced with the rainy day.

% 1. check dependency NSUBJ(verb, noun), the verb is matched to a transformation name based on word2vec; the noun is matched to an ontology element.
% 2. check all dependencies of the subject, identify properties and set them to an ontology instance.
% 3. check all dependencies of the verb, identify transformation parameters based on predicate logic. 
With this ontology, {\tool} matches all ontology elements in dependency predicates of the ``If'' clause. First, the parser checks the dependency predicate {\em NSUBJ(noun, verb)} to identify the ontology element (the noun) and the transformation on the element (the verb). Then for the subject noun, the parser analyzes all related predicates of it such as the {\em amod(adj, noun)} and {\em advmod(adv, noun)} because these dependencies show modifiers on the subjective noun, which are corresponding to properties of the ontology element. Then for identified adjectives and adverbs in these predicates, the parser converts them to vectors using word2vec and then matches them with predefined ontology property vectors. Specifically, we calculate the distance of an adjective to all predefined properties of the element. The minimal distance is identified and the corresponding predefined property is possibly the correct property described in the rule. We further check whether the minimal distance is over a predefined threshold to eventually identify the property of the ontology element. In the previous example, the dependency predicate {\em NSUBJ(pedestrian, appears)} is first identified and the subjective noun {\em pedestrian} is matched to the ontology element \textbf{Pedestrian}.     

For identifying the transformation, the parser extracts the verb in the dependency predicate {\em NSUBJ(noun, verb)} and convert it to a vector using word2vec. Then it is matched with predefined transformations based on the minimal distance of vectors. In the example, the verb {\em appear} is extracted and matched with the transformation {\em Add}. For transformations, another problem is to identify their parameters. For example, for {\em Add} transformation it requires the position to add an element and for {\em Replace} transformation it needs to know which element is used to replace the current one. To solve this problem, the parser analyzes the indirect dependency between the verb and a noun defined by a preposition such as {\em on(noun, verb)}. The extracted noun is then matched to the parameter of the transformation. In the example, {\em roadside} is extracted from the dependency predicate {\em on(roadside, appear)} and identified as the position to add a pedestrian. A new predicate {\em Add(pedestrian, roadside, on)} is created, where the {\em pedestrian} is the ontology element with its properties. Table~\ref{tab:predicate} shows the translations of three transformations with their parameters.
The parser checks whether a few predicates exist simultaneously and then infer to the corresponding transformation predicate.

\begin{table*}[]
\centering
\caption{Predicate translations for transformations}
\label{tab:predicate}
\renewcommand{\arraystretch}{1.4}

\begin{tabular}{|l|l|}

\hline
\multirow{3}{*}{\textbf{Add}}     & NSUBJ(\(n_1\), v) \(\wedge\) ONTOLOGY(\(n_1\)) \(\wedge\) TRANSFORMATION(v, add) \(\wedge\) ON(\(n_2\), v) \(\wedge\) POSITION(\(n_2\)) \(\rightarrow\) ADD(\(n_1\), \(n_2\), on)                                                                                                                      \\ \cline{2-2} 
                                  & NSUBJ(\(n_1\), v) \(\wedge\) ONTOLOGY(\(n_1\)) \(\wedge\) TRANSFORMATION(v, add) \(\wedge\) FRONT(\(n_2\), v) \(\wedge\) ONTOLOGY(\(n_2\)) \(\rightarrow\) ADD(\(n_1\), \(n_2\), front)                                                                                                                \\ \cline{2-2} 
                                  & NSUBJ(\(n_1\), v) \(\wedge\) ONTOLOGY(\(n_1\)) \(\wedge\) TRANSFORMATION(v, add) \(\wedge\) BEHIND(\(n_2\), v) \(\wedge\) ONTOLOGY(\(n_2\)) \(\rightarrow\) ADD(\(n_1\), \(n_2\), behind)                                                                                                              \\ \hline
\textbf{Remove}                   & NSUBJ(n, v) \(\wedge\) ONTOLOGY(n) \(\wedge\) TRANSFORMATION(v, remove) \(\rightarrow\) REMOVE(n)                                                                                                                                                                                    \\ \hline
\multirow{2}{*}{\textbf{Replace}} & \begin{tabular}[c]{@{}l@{}}NSUBJ(\(n_1\), v) \(\wedge\) ONTOLOGY(\(n_1\)) \(\wedge\) TRANSFORMATION(v, replace) \(\wedge\) PREP(\(n_2\), v) \(\wedge\) ONTOLOGY(\(n_2\)) \(\wedge\) \\ WEATHER (\(n_2\)) \(\wedge\) WEATHER(\(n_2\)) \(\rightarrow\) REPLACE(\(n_1\), \(n_2\), weather)\end{tabular} \\ \cline{2-2} 
                                  & \begin{tabular}[c]{@{}l@{}}NSUBJ(\(n_1\), v) \(\wedge\) ONTOLOGY(\(n_1\)) \(\wedge\) TRANSFORMATION(v, replace) \(\wedge\) PREP(\(n_2\), v) \(\wedge\) ONTOLOGY(\(n_2\)) \(\wedge\) \\ OBJECT (\(n_1\)) \(\wedge\) OBJECT(\(n_2\)) \(\rightarrow\) REPLACE(\(n_1\), \(n_2\), object)\end{tabular}    \\ \hline
\end{tabular}
\end{table*}

% First, {\tool} checks dependency tuples that describes dependencies between a noun and a verb because the verb is most likely the transformation for applying and the subject noun is the ontology element to be transformed. When verbs in dependency tuples are identified, {\tool} converts them to vectors via Word2vec technique~\cite{}. Then {\tool} calculates distances between these vectors and vectors of predefined transformations {\em Add, Remove, Replace}. The pair (verb, transformation) with the minimal distance is identified. The related noun is then identified and matched with ontology elements. Once the verb for transformation and the noun for an ontology element are identified, {\tool} travels all dependency tuples of them and matches properties of the ontology element.

% In the previous example, the only verb {\em appear} and its dependency tuple {\em (pedestrian, appear)} are first identified. By calculating the distance between the word appear and three transformations, {\tool} finds the closest distance between {\em appear} and {\em Add}. Therefore, {\tool} identifies the transformation to be applied is {\em Add.} Then {\tool} extracts {\em pedestrian} from the dependency tuple {\em (pedestrian, appear)} and matches it with elements in the ontology. Finally, {\tool} travels all dependency tuples of {\em pedestrian} and {\em appear}. The word {\em roadside} is found and matches with the property {\em position} of the pedestrian element. When all properties are extracted, an ontology entity of pedestrian with a property position roadside is thus initialised. {\tool} then sends the ontology entity and the transformation to be applied to the test generator for synthesis new driving images.
For ``Then'' clause, the parser follows the same process to identify the expected change as the verb in the predicate {\em NSUBJ(noun, verb). The extracted verb then is matched to predefined expected change {\em increase}, {\em decrease} and {\em keep}. The parser further traversing dependency predicates of the verb to get the detail of the expected change. In the example, {\em npadvmod(30\%, slow)} and {\em advmod(30\%, least)} are identified. The parser then infer that speed should decrease at least 30\%.}
% For ``Then'' clause, {\tool} aims to identify key information {\em expected change}, which describes in the new driving image how the behavior of ego-vehicle such as speed and steering angle should change (increase, decrease, or keep the same) to what extent. Following the same procedure, {\tool} first checks the verb in dependency tuples and then convert it to a vector. Then the distance between the verb and three pre-defined expected changes {\em increase, decrease,} and {\em keep}. {\tool} further travels dependency tuples of the verb to identify the extent of the expected change. In the above example, {\em slow} is identified and thought as the expected change {\em decrease}. Then from the dependency {\em (slow, down at least 30\%)}, {\tool} knows the extent of speed decrease.     

% how to extract information from then clause

% When key information are extracted from the ``If'' statement in the testing rule, {\tool} uses a driving scenario ontology to match the information and creates an ontology entity that is used to guide the generation of new driving scenarios in the test generator.

% Ontology is a methodology to formally summarize categories and create a knowledge base to organize properties and relations in a specific domain. Ontology has been used to model traffic conditions and driving scenarios in previous work~\cite{}. Inspired by these prior work, we propose to use ontology for modeling elements that could be changed and affect driving behaviors. Specifically, we define ontologies that contain three categories of elements. For each category, it contain several classes and sub-classes. Finally, an ontology entity of a class could be initialized by setting its properties.

% Figure~\ref{fig:ontology} shows a subset of the proposed ontology in hierarchy. In the second layer, three categories are road, object, and weather and time. For each category, possible classes of elements are demonstrated in the third layer. For example, in the category object, the possible elements could be vehicles and pedestrians. A vehicle could be described more accurately as a car or a school bus entity, as the fourth layer shown. Finally, we can set properties of entities such as setting the position and color of a car entity. 

% In the previous example, when information {\em pedestrian} and {\em on the roadside} are extracted, a pedestrian ontology entity with position property on the road side could be generated. Then the ontology entity and extracted transformation are sent to the test generator to create new driving scenario images.

% An entity defined by the ontology could be described in natural language. For example, if we say ``A white car appears in the front of the ego vehicle'', we actually define a car entity with the properties position ``in the front'' and color ``white''. ``Appear'' is corresponding to the relation {\em add}. Therefore, we describe how to use an ontology entity to change the current scenario. In natural language, the description of the properties of an entity could be pretty flexible. 

% In the ontology, now we define four kinds of relations including \textit{Add}, \textit{Remove}, \textit{Update} and \textit{Replace} to transform the current scenario. The \textit{Add} relation 
% can be used to add an entity into current scenario. For the \textit{Update} relation, it could update weather and time of the current scenario. For the \textit{Replace} relation, it can be used to change an entity to another one in the current scenario (e.g.,  replacing \textit{Buildings} to \textit{Trees}.
% The \textit{Remove} relation can remove an entity from the driving scenario.
}


% When all values of rule components in the input rule are extracted, the parser will also validate whether the user-input values match with predefined values for each rule component, which is stored in a configuration file. 

% When these rule components are validated, the rule components from “If” statement(s) are

% passed to the metamorphic test generator which is used to select the corresponding transformation engine for test cases generation. Rule components extracted from  ``Then" statement(s) are used to form MR(s).


{\color{blue}
\subsubsection{Metamorphic relation generation}
%When rule components \textit{Target action}, \textit{Expected change} and \
%\textit{Change parameter} are extracted, they could be used to create an MR mathematically,

When {\em ontology element}, {\em transformation}, and {\em expected change} are obtained from the testing rule, {\tool} creates an MR based on them. Let the original driving image be \(x_o\), the ontology entity be \(O\), the transformation be \(T\), the test generator be \(G\), the driving model under test be \(F\), Then the new driving image is represented as \(G(x_o, O, T)\), and model predictions on two driving images are \(F(x_o)\) and \(F(G(x_o, O, T))\).
Then an MR is represented by an expected change function \(E\) that takes two model predictions as inputs, as shown in Formula \ref{eq:mr}. 
% which checks whether the output of \(E\) is 1. If not, model predictions on the original driving image and the new driving image violates the MR.
\begin{equation}
\label{eq:mr}
  E(F(x_o), F(G(x_o, O, T)))
\end{equation}

The build block of the expected change function is \(F(x_o) - F(G(x_o, O, T)\), which describes the difference between two model predictions. Then based on the expected change and the extent of change in the extracted information, the expected change function is created. 
In the previous example, the expected change is {\em decrease} and the extent of change is {\em at least 30\%}, which is thus transferred to the function \((F(x_o) - F(G(x_o, O, T))) / F(x_o) >= 30\% \). If the extent of change is not presented as a percentage but a number as the example ``decrease 10 km/h'', then the expected change function is \(F(x_o) - F(G(x_o, O, T) >= 10 \). If the user does not describe the extent of the change, then the default value is 0 and the function is \(F(x_o) - F(G(x_o, O, T) >= 0 \). For the expected change {\em increase}, the creation of the expected change function is similar. For the expected change {\em keep}, considering the change of input image would change the model prediction to some extent, we follow the same setting in ~\cite{zhang2018deeproad}, and generate the function as \(|F(x_o) - F(G(x_o, O, T)| < \epsilon \) where \(\epsilon\) is a small threshold.
}

% When (\textit{Target action}, \textit{Expected change} and 
% \textit{Change parameter}) are extracted from ``Then" statement(s), they are used to create the MR(s) in mathematical formulas to describe the relationship between the model prediction of the source test case and that of the follow-up test case. Let a source test case be \(x_o\), the transformation be \(G\), and transform parameters be \(p\). The follow-up test case can be presented as \(G(x_o, p)\). Given the driving model under test \(F\), two model predictions can be presented as \(F(G(x_o, p))\) and \(F(x_o)\).  

% {\color{red}TODO: add a formula for describing MRs}


% In Rules 1-3, \textit{Decrease} is the input value for \textit{Expected change},  an MR \(F(G(x_o, p)) - F(x_o) < 0\) can thus be created. In Rule 4, \textit{At least 30\%} is provided for \textit{Change parameter}, the corresponding MR is \(F(G(x_o, p))/F(x_o)<1-0.3\). In Rules 6 and 7, 
% \textit{Keep the same} is provided for \textit{Expected change}, 

% considering the change of input image would change the model prediction to some extent, we follow the same setting in ~\cite{zhang2018deeproad}, and generate the MR as \(|F(G(x_o, p) - F(x_o)| < \epsilon \) where \(\epsilon\) is a small threshold. 

% For complicated rules such as Rule 5, two follow-up cases \(G(x_o, p_1)\) and \(G(x_o, p_2)\) are generated. Two %metamorphic relations
% MRs described in two ``Then..." statements are thus created with the first one ``Then the speed of ego-vehicle should decrease"  denoted by \(F(G(x_o, p_1)) - F(x_o) < 0\) and the second ``Then" statement represented by \(F(G(x_o, p_2)) - F(G(x_o, p_1)) < 0\).
% When two MRs are used in the same rule, failure of one MR means the entire test case fails.


%Both two MRs should be passed at the same time. If any MR is not held in the test, the test case is failed.


% For Rules 1-3, the created MR is Formula~\ref{eq:mr_1}; For Rule 4, the created MR is Formula~\ref{eq:mr_2}; For Rule 5, the created MR is Formula~\ref{eq:mr_3}; For Rule 6-7, the created MR is Formula~\ref{eq:mr_4}. The setting of \(\epsilon\) is introduced in Section~\ref{sec:experiment}. 

% \begin{equation}
% \label{eq:mr_1}
%   F(G(x_o, p) - F(x_o) < 0 
% \end{equation}
% \vspace{-15pt}
% \begin{equation}
%   (F(x_o) - (F(G(x_o, p)) / F(x_o) >= 30\% \label{eq:mr_2}
% \end{equation}
% \vspace{-15pt}

% \begin{equation}
% \label{eq:mr_3}
% \begin{cases}
%     F(G(x_o, p_1) - F(x_o) < 0, \\
%     F(G(x_o, p_2) - F(x_o, p_1) < 0 \\
% \end{cases} 
% \end{equation}
% \vspace{-15pt}

% \begin{equation}
%   \left| F(G(x_o, p) - F(x_o)) \right| < \epsilon \label{eq:mr_4}
% \end{equation}

{\color{blue}
\subsection{Metamorphic Test Generator}
\label{sec:MT generator}

The test generator creates new driving images based on the transformation predicate that contains the transformation name, transformation subject (ontology element), and transformation parameters. For different transformation and ontology element, the test generator applies different image generation techniques including image manipulation, image synthesis, and image-to-image translation. 

\subsubsection{Image manipulation}
We implement the image manipulation based on semantic label maps and use the technique to add ontology elements into driving images. A semantic label map is the ground truth of semantic segmentation task that aims to perceive the driving environment. Given an driving image, the corresponding semantic label map provides image classification results in pixel level. In this work, we assume the test driving dataset contains annotated semantic label maps of driving images. As Figure~\ref{fig:semantic_label_map} shows, image (a) is the driving scene, and image (b) is the semantic label map associating each pixel in the image (a) with a class of different color (e.g., the blue area in the semantic label map represents the sky in the original image).  Based on the semantic label map, we are able to extract an object belonging to a class (aka the mask) from the original image, as shown in image (c). We use OpenCV~\cite{opencv_library} to identify the exact position of different objects and extract object masks as templates.

In this way, we create a template pool for ontology entities (e.g., a pedestrian on the roadside or a black car in the front of the ego-vehicle) by looking through the testing set to extract templates and annotate them as ontology entities. To add an ontology element into driving images, {\tool} first matches the ontology element with its template mask in the template pool. Then {\tool} adds the mask into the driving images using OpenCV. In the previous example, the ontology element is {\em a pedestrian} and the transformation parameter is {\em roadside}. Therefore, the corresponding template mask is selected and added into test images. A problem is for different images the position of the roadside are possible different. We solve this problem by checking the boundary of the road by semantic label map of the target image. More specifically, we move the mask horizontally by changing the x-axes coordinates of the mask and then check whether at the current position of the mask, the semantic label of the left bottom pixel is changing from road to other class. If so, we add the mask at that position.

\subsubsection{Image synthesis}
We implement the image synthesis technique based on a generative model called {\em Pix2pixHD}~\cite{wang2018high}. {\tool} applies the model to remove and replace ontology entities belonging to categories road or object. Pix2pixHD is a Generative Adversarial Network (GAN)~\cite{goodfellow2014generative} for image generation based on semantic label maps. Given a semantic label map of a driving scene image, {\em Pix2pixHD} synthesizes the corresponding driving scene image (e.g., generating Figure~\ref{fig:semantic_label_map}(a) based on~\ref{fig:semantic_label_map}(b)). For example, if the ontology entity is ``dashed lane lines'' and the transformation is ``Remove'', the test generator detects pixels in the semantic label map with the class as dashed lines and then change the label of these pixels to road. Similarly, if the user wants to replace the buildings in the driving images to trees, the test generator changes the pixels of buildings in the semantic label to trees. Then the test generator calls Pix2pixHD to generate a new driving image based on the modified semantic label map.   

\subsubsection{Image-to-image translation}
To implement the {\em Replace} transformation on ontology entities belonging to the category {\em Weather \& Time}, we use another image-to-image translation GAN called UNIT~\cite{liu2017unsupervised}. The main function of {\em UNIT} is to transform images from one domain to another (e.g., changing a tiger to a lion). We integrate pre-trained models of {\em UNIT} on BDD100K~\cite{yu2018bdd100k} for transforming images to different weather conditions and driving time.


\subsubsection{Image filter}
When generating new driving images, not all testing images are qualified to be transformed. For example, if the user wants to add a vehicle in the front of the ego-vehicle but there is already a vehicle or other objects at the same position in the testing image, such images should be filtered out. Therefore, we apply a test case filter mechanism within image transformation techniques. For adding an ontology entity, we check whether another object also exists at the position to put the mask. For removing and replacing an ontology, we check whether the number of pixels belonging to the class to be replaced takes account a certain percentage of the number of all pixels in a semantic label map. The filter is set to avoid conditions where generated new images are pretty similar as the original driving image. For replacing weather and driving time, we filter generated driving images that have small L2 distances to original driving images because in this condition the original driving images are most possibly already in the target weather or driving time.     

\begin{figure*}
\centering
\subfloat[The original image]{\includegraphics[width=.3\textwidth]{images/original2.png}\label{fig:rule5_1}}\hfil
\subfloat[The image after segmentation]{\includegraphics[width=.3\textwidth]{images/segment2.png}\label{fig:rule5_2}}\hfil
\subfloat[The segmented vehicle]{\includegraphics[width=.3\textwidth]{images/vehicle2.png}\label{fig:rule5_2}}\hfil 
\caption{An example of image segmentation}\label{figure}
\vspace{-6pt}
\label{fig:semantic_label_map}
\end{figure*}
}

% \subsubsection{Image Manipulation}
% {\color{blue}
% Image manipulation is a task to modify images such as adding or removing an object while keep the fidelity of other objects and scenes. In this paper, we implemented two generators for image manipulation: a template-based image manipulation generator and a generative model. Both of them rely on semantic segmentation and semantic label maps.

% Semantic segmentation is essential for autonomous driving by perceiving the driving environment. Given an image, semantic segmentation aims to generate a semantic label map that provides image classification results in pixel level. Several datasets for autonomous driving such as Cityscapes~\cite{cordts2016cityscapes}, A2D2~\cite{geyer2020a2d2}, and BDD100K~\cite{yu2018bdd100k} provide driving scene images and corresponding semantic label maps. As Figure~\ref{fig:semantic_label_map} shows, image (a) is the driving scene, and image (b) is the semantic label map associating each pixel in the image (a) with a class of different color (e.g., the blue area in the semantic label map represents the sky in the original image). Based on the semantic label map, we can extract an object belonging to a class (aka the mask) from the original image, as shown in image (c). We used OpenCV~\cite{opencv_library} to identify the exact position of different objects and extracted object masks as templates. Then we can add these object masks into any images.  

% We first look through the original dataset and create a template database to store masks of different objects (e.g., pedestrians at different locations). For example, we first find a reference image where a pedestrian is located at the roadside. With the semantic label map of the reference image, we can obtain the accurate shape and location of an object with class label ``pedestrian'' and then extract a mask of this pedestrian from the reference image. The mask stores information about the appearance of the pedestrian and the coordinates of each pixel belonging to the pedestrian. Therefore, when the scenario ontology requires to add a person, the corresponding template mask will be selected and added on an original image. A problem is for different images the position of the roadside are possible different. We solve this problem by checking the boundary of the road by semantic label map of the target image. More specifically, we move the mask horizontally by changing the x-axes coordinates of the mask and then check whether at the current position of the mask, the semantic label of the left bottom pixel is changing from road to other class. If so, we add the mask at that position.




% When manipulating attributes of the scenario ontology entity, semantic label maps are also helpful for identifying properties like position and heading of an object. In the above example, the ontology entity pedestrian has a property location {\em on the roadside}. To ensure the extracted pedestrian from the template base can be added on the roadside in the target image, we check the boundary of the road by semantic label map of the target image. Therefore, we move the mask horizontally by changing the x-axes coordinates of the mask to find the end of the road by checking the semantic label of the left bottom pixel of the mask changing from road to other class.


% In addition, we applied a generative model called {\em Pix2pixHD}~\cite{wang2018high} for generating modified images. Pix2pixHD is a Generative Adversarial Network (GAN)~\cite{goodfellow2014generative} for image generation based on semantic label maps. For example, given a semantic label map of a driving scene image, {\em Pix2pixHD} could synthesize the corresponding driving scene image (e.g., generating Figure~\ref{fig:semantic_label_map}(a) based on~\ref{fig:semantic_label_map}(b)). Therefore, when we change the input semantic label maps, {\em Pix2pixHD} could create a corresponding new image. 

% To implement Remove and Replace Transformations, we first modify images' semantic label maps and then use {\em Pix2pixHD} to generate images. For example, if a scenario ontology is ``removing dashed lane lines from the road'', we first detect pixels in the semantic label map with the class as dashed lines. Then we change the label of these pixels as road.

% For replacing buildings with trees, we similarly change the label of pixels from the building to the tree. A built-in filter is implemented in this transformation engine to filter images that the number of pixels belonging to lines is less than 1\% (Rule 6) or belonging to buildings is less than 5\% (Rule 7) of the number of all pixels in a semantic label map. The filter is set because it is difficult to find the target object lane lines or buildings in such images.

% \subsubsection{Image-to-image Translation}
% Image-to-image translation is a technique to generate an image based on another image in another domain or another style. To implement Update transformation on weather and time scenario ontologies, we applied a GAN called {\em UNIT~\cite{liu2017unsupervised}} for this. The main function of {\em UNIT} is to transform images from one domain to another (e.g., changing a tiger to a lion). We integrated pre-trained models of {\em UNIT} on BDD100K~\cite{yu2018bdd100k} for transforming images to other weather conditions. 


% }
% \textbf{Integrating OpenCV} - 
% OpenCV~\cite{opencv_library} is a powerful library for image processing. It supports image manipulation at the pixel level. We integrate {\em OpenCV} for Add transformation in Rules 1, 2, 4, and 5 based on semantic label map and template-based image manipulation~\cite{wang2018high} that uses predefined templates of different object masks to modify the original image. 

% As Figure~\ref{fig:semantic_label_map} shows, image (a) is the driving scene, and image (b) is the semantic label map associating each pixel in the image (a) with a class of different color (e.g., the blue area in the semantic label map represents the sky in the original image). Based on the semantic label map, we can extract an object belonging to a class (aka the mask) from the original image, as shown in image (c). Semantic segmentation is essential for autonomous driving by perceiving the driving environment. Several datasets for autonomous driving such as Cityscapes~\cite{cordts2016cityscapes}, A2D2~\cite{geyer2020a2d2}, and BDD100K~\cite{yu2018bdd100k} provide driving scene images and corresponding semantic label maps. To implement the transformation required in Rules 1 and 4 (``Add a pedestrian at the roadside''), we first look through the original dataset and find a reference image where a pedestrian is located at the roadside.
% With the semantic label map of the reference image, we can obtain the accurate shape and location of an object with class label ``pedestrian'' and then extract a mask of this pedestrian from the reference image. The mask stores information about the appearance of the pedestrian and the coordinates of each pixel belonging to the pedestrian. Then we can use {\em OpenCV} to add this mask on a target image to generate a transformed image as required. To ensure the extracted pedestrian is still located at the roadside in the target image, we need to identify the roadside location.
% As roadside is not annotated as a class in the dataset used, intuitively we regard the boundary of the road as the roadside.
% Therefore, we move the mask horizontally by changing the x-axes coordinates of the mask to find the end of the road by checking the semantic label of the left bottom pixel of the mask changing from road to other class. To avoid newly identified class is somewhere we still cannot add a pedestrian onto (e.g., there is a car at the position so we cannot add a pedestrian), 
% a built-in filter is implemented to directly filter out those images where required transformation is not possible.
% Similarly, to add a pedestrian closer to the ego-vehicle (Rule 5), we first vertically move the pedestrian mask down $50$ pixels and scale up the size of the mask to 1.5 times than the original one. The scale ratio is obtained by referring to the size of other objects at the same location in the given dataset. Then we follow the same procedure to add the mask at the roadside. To implement the transformation required in Rule 2 (``Add a slow speed sign at the roadside''), we follow the same procedure to extract a mask of a slow speed sign from a reference image and add it at the roadside.


% \textbf{Integrating UNIT} - 
% UNIT~\cite{liu2017unsupervised} is a neural network based on Generative Adversarial Networks (GANs)~\cite{goodfellow2014generative} and Variational Autoencoders (VAEs)~\cite{kingma2019introduction} for image-to-image translation. The main function of {\em UNIT} is to transform images from one domain to another (e.g., changing a tiger to a lion). In this paper, we use {\em UNIT} as an engine in {\tool} to implement Update transformation to change the driving scene to night (Rule 3). To do this, we directly used a pre-trained model. A built-in filter is implemented in this transformation engine to filter images that already contain a nighttime driving scene by judging whether the pixels extracted from the background area (normally the top center area of an image) are close to the black color. 

% \textbf{Integrating Pix2pixHD} - 
% Pix2pixHD~\cite{wang2018high} is an image-to-image translation technique proposed by Nvidia for generating and manipulating images based on the semantic label maps. For example, given a semantic label map of a driving scene image, {\em Pix2pixHD} could synthesize the corresponding driving scene image (e.g., generating Figure~\ref{fig:semantic_label_map}(a) based on~\ref{fig:semantic_label_map}(b)). Therefore, when we change the input semantic label maps, {\em Pix2pixHD} could create a corresponding new image. We use {\em Pix2pixHD} as an engine to implement Remove and Replace Transformations {\em Rules 6-7}. For removing lane lines from the road, we first detect pixels in the semantic label map with the class as dashed lines or solid lines. Then we change the label of these pixels as road. For replacing buildings with trees, we similarly change the label of pixels from the building to the tree.
% A built-in filter is implemented in this transformation engine to filter images that the number of pixels belonging to lines is less than 1\% (Rule 6) or belonging to buildings is less than 5\% (Rule 7) of the number of all pixels in a semantic label map. The filter is set because it is difficult to find the target object lane lines or buildings in such images.




\begin{comment}


\subsection{Configuration file}
\label{sec:configration}
% The configuration file records each transformation engine as well as its ability what transformations it can implement and which objects it can manipulate. By matching the configuration and elements, the correct transformation engine is thus selected. 
% Due to the decoupling design of configuring transformation engines in the configuration file, it is easy to integrate other transformation engines into {\tool}
%The prototype of 
{\tool} adopts an XML configuration file to manage and coordinate components of {\tool} framework. Specifically, the configuration file stores all available values of rule template components, the setting of each available transformation engine, and information regarding available driving models and testing dataset.

Figure~\ref{fig:config} shows a subsection of the configuration file for specifying a transformation engine. In the sample given, we specify the name of the transformation engine (e.g., {\em OpenCV}), the python library for the implementation (e.g., opencv\_gen.py), and what transformation this engine is enabled (e.g., add) along with supported objects (e.g., pedestrian and slow speed sign) in the driving scenes which this transformation can be performed with. Such setting allows flexible extension of {\tool}. For instance, if we need a new transformation engine for object injection, we can simply replace the ``OpenCV'' with the new transformation engine name and update ``entry'' with the implementation of the new engine. If we implement a new transformation engine that supports adding other objects such as vehicles, we can also integrate it into {\tool} by changing both the \textit{entry} attribute to the new transformation and the attribute of \textit{support object}.  {\tool} does have a requirement that for each transformation implementation, it needs to implement a mandatory function which takes parameters required for the transformation (e.g., Object and Transformation parameters) and generates required transformed images.

\end{comment}

%{\color{red}provides a function called ``Image control'' taking rule components Object and Transform parameters as function parameters for image manipulation}

%The third node defines a transformation engine called OpenCV, the entry for calling the transformation engine in python code that implements an interface \textit{image control}, and a nested node \textit{support transformation} with its \textit{supported objects}. The metamorphic test generator chooses the correct transformation engine by matching the support transformation with extracted value of transformation from the rule template. In the configuration file, it is convenient for testers to add or modify transformation engines, which makes {\tool} more extensible. {\color{red}For example, If we implement a better transformation engine for Add transformation on objects pedestrian and speed slow sign , we can simply replace it with current OpenCV transformation engine by changing the engine name ``OpenCV'' to the new name and update the value of entry. If we implement a new transformation engine for Add transformation on other objects such as vehicles, we can also integrate it into {\tool} by following the definition of OpenCV transformation engine but change the attribute \textit{support object} of the nested node \textit{support transformation}. }

%{\color{red}For example, If we implement a better transformation engine for Add transformation on objects pedestrian and speed slow sign , we can simply replace it with current OpenCV transformation engine by changing the engine name ``OpenCV'' to the new name and update the value of entry. If we implement a new transformation engine for Add transformation on other objects such as vehicles, we can also integrate it into {\tool} by following the definition of OpenCV transformation engine but change the attribute \textit{support object} of the nested node \textit{support transformation}. }

\begin{comment}
Figure~\ref{fig:config} shows examples of configuration about the keyword transformation in the rule template and the setting of a transformation engine. The first node defines an object %called
named pedestrian. The second node defines a transformation named add. The attribution {\em support\_object} declares that the transformation can apply to which objects. The attribution {\em parameter} is corresponding to the rule component \textit{transformation parameter}. After the values of rule components in the rule template are extracted by the rule parser, the rule parser will validate extracted components by matching predefined keywords of all rule components in the configuration file. First, it validates whether all extracted values of rule components are defined in the configuration file. If not, the input testing rule is not supported by the prototype. Second, it validates whether extracted value of object is in the predefined support object in the transformation node. If not, the needed transformation in the testing rule is also not supported now. In these cases, the testing is terminated. 

The third node defines a transformation engine called OpenCV, the entry for calling the transformation engine in python code that implements an interface \textit{image control}, and a nested node \textit{support transformation} with its \textit{supported objects}. The metamorphic test generator chooses the correct transformation engine by matching the support transformation with extracted value of transformation from the rule template. In the configuration file, it is convenient for testers to add or modify transformation engines, which makes {\tool} more extensible. {\color{red}For example, If we implement a better transformation engine for Add transformation on objects pedestrian and speed slow sign , we can simply replace it with current OpenCV transformation engine by changing the engine name ``OpenCV'' to the new name and update the value of entry. If we implement a new transformation engine for Add transformation on other objects such as vehicles, we can also integrate it into {\tool} by following the definition of OpenCV transformation engine but change the attribute \textit{support object} of the nested node \textit{support transformation}. }
\end{comment}
% \jzcomment{I think the configuration part is fine, but what is important to make clear here is with the provided framework, when users need to provide such configuration files? for every single rule? It is not clear now. It is important to judge how automated the framework is. I think it is fine to configure for every single rule so long afterwards the test generation is automated. Another question is how to plug-in a new transformation (e.g., snow weather or desert scene), I guess just need to specify an entry in [engine] subsection? can you be more specific of the concrete steps invovled in adding a new transformation engine. The introduction for openCV is not very clear}

% With the configuration file, {\tool} can load necessary information about keywords in the rule template to help parse input rules and information about transformation engines to help apply the correct transformation on objects.



% \begin{figure}[ht]
% \centering
% \includegraphics[width = .5\textwidth]{images/rmt_configuration_2.png}
% \caption{A configuration example}
% \label{fig:config}
% \end{figure}

\subsection{Metamorphic Relation Evaluator}
When new driving images are generated and unqualified images are filtered out, a metamorphic testing set containing source test cases (original driving images) and follow-up test cases (generated new driving images) is created. Then the metamorphic relation evaluator feeds the metamorphic testing set into the driving model under test and obtains model predictions. Finally, the evalutor uses the created MR to validate each prediction pair (prediction 1 for an image from
source test cases, prediction 2 for the corresponding transformed images from 
follow-up test cases). If the prediction pair violates the MR, a violation (erroneous behavior) of the driving model is detected.

% When the input rule is successfully parsed and the correct transformation engine is selected, the metamorphic relation evaluator will call the test generator transformed test set based on original test set. 
% During the process, the transformation engine filters images
% unqualified to be transformed. Then the source and follow-up test cases are fed into the driving model under test. The predictions for the original test set and the predictions for the follow-up test set are obtained. Finally, the evaluator would use the MR created by the NLP-based parser to validate each prediction pair (prediction 1 for an image from %the original test set
% source test cases, prediction(s) 2 for the corresponding transformed images from %the follow-up test set
% follow-up test cases. If the prediction pair violates the MR, a violation (erroneous behavior) of the driving model is detected.

% The evaluator is used to validate whether the prediction pairs \(<f(x), f(g(x, 0))>\) have the relationship defined by the underlying MR. A defect is found if the prediction pair violates the MR. 

\subsection{Implementation}
We implement a prototype of {\tool} to support the generation of metamorphic testing sets and detect anomaly behaviors of driving models.
%that implements three components described before to test driving models. 
%Now the prototype can support seven proposed rules.
Figure~\ref{fig:gui_main} shows the main GUI of the prototype. In the text box, a tester could input the testing rule. Then the tester only needs to select the model under test and the testing dataset. The prototype can automatically parse the rule, create the MR, generate source and follow-up test cases, and detect violations. Then a window like Figure~\ref{fig:gui_result} will pop up to show the testing result. The first line of text tells the number of detected violations and the total number of generated test cases (e.g., $294$ violations were found out of $532$ test cases). A sample of detected violations is shown in the middle of the popup window. The left image in the picture shows the original test case and the driving model prediction on the image. The right image shows the transformed image as well as the model prediction on it. By comparing the predictions, the tester can verify whether the MR is indeed violated. Finally, a line of text at the bottom tells the tester the storage path of images for all detected violations. 

\begin{figure}[ht]
\centering
\includegraphics[width = .47\textwidth]{images/rmt_gui_ase.png}
\caption{The main interface for specifying traffic rules in {\tool}}
\label{fig:gui_main}
\end{figure}

\begin{figure}[ht]
\centering
\includegraphics[width = .45\textwidth]{images/rmt_result_addbox.png}
\caption{A sample of detected traffic rule violations for user inspection. A pedestrian is added on the roadside while the ego-vehicle does not slow down.}
\label{fig:gui_result}
\end{figure}




==> result.tex <==
\section{Evaluation}
\label{sec:results}
Figure~\ref{fig:pix2pix_generate} shows the generated metamorphic driving scenes from the underlying five rules. In this section, we will analyze how well these scenes generated from rule-based MRs can detect faults in Section~\ref{subsection:RQ1}, how thresholds for these rules can impact fault detection in Section~\ref{subsection:RQ2}, and how truthful are the faults detected by experienced human judges in Section~\ref{subsection:RQ3}.


\begin{figure*}

\centering
\subfloat[Original driving scene]{\includegraphics[width=.17\textwidth]{images/car_original.jpg}\label{fig:generate_a}}\hfil
\subfloat[Original driving scene]{\includegraphics[width=.17\textwidth]{images/bicycle_original.jpg}\label{fig:generate_b}}\hfil 
\subfloat[Original driving scene]{\includegraphics[width=.17\textwidth]{images/person_original.jpg}\label{fig:generate_c}}\hfil 
\subfloat[Original driving scene]{\includegraphics[width=.17\textwidth]{images/night_original.jpg}\label{fig:generate_d}}\hfil 
\subfloat[Original driving scene]{\includegraphics[width=.17\textwidth]{images/rainy_original.jpg}\label{fig:generate_e}}\hfil 

\subfloat[Adding a car]{\includegraphics[width=.17\textwidth]{images/car_add.jpg}\label{fig:generate_f}}\hfil   
\subfloat[Adding a bicycle]{\includegraphics[width=.17\textwidth]{images/add_bicycle.jpg}\label{fig:generate_g}}\hfil
\subfloat[Adding a pedestrian]{\includegraphics[width=.17\textwidth]{images/person_add.jpg}\label{fig:generate_h}}\hfil
\subfloat[Day2night]{\includegraphics[width=.17\textwidth]{images/night_add.jpg}\label{fig:generate_i}}\hfil
\subfloat[Normal2rainy]{\includegraphics[width=.17\textwidth]{images/rainy_add.jpg}\label{fig:generate_j}}\hfil
\caption{Examples of source test cases and follow-up test cases for five rules}\label{figure}
\vspace{-6pt}
\label{fig:pix2pix_generate}
\end{figure*}


\subsection{RQ1: Fault Detection Capability}
\label{subsection:RQ1}
% {\color{red}subsection 1: results of fault coverage for each metamorphic relation}
% {\color{blue} and  }
% {\colr{red}Huai -- I think ``fault detection sensitivity'' is more accurate than ``fault coverage'' as the title for this subsection.}
% \begin{figure}[htbp]
% \centering
 
% \subfigure[]{
%     \begin{minipage}[t]{1\linewidth}
%         \centering
%         \includegraphics[width=.5\textwidth]{images/rule-1.png}\\
%         \vspace{0.02cm}
%         \includegraphics[width=.5\textwidth]{images/rule-2.png}\\
%         \vspace{0.02cm}
%         \includegraphics[width=.5\textwidth]{images/rule-3.png}\\
%         \vspace{0.02cm}
%         \includegraphics[width=.5\textwidth]{images/rule-4.png}\\
%         \vspace{0.02cm}
%         \includegraphics[width=.5\textwidth]{images/rule-5.png}\\
%         \vspace{0.02cm}
%         %\caption{fig1}
%     \end{minipage}%
% }%

% \end{figure}
% \begin{figure}[ht]
% \centering
% \includegraphics[width =.5\textwidth]{images/rule-1.png}
% \caption{Fault detection sensitivity of rule 1}
% \label{fig: rule-1}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width =.5\textwidth]{images/rule-2.png}
% \caption{Fault detection sensitivity of rule 2}
% \label{fig: rule-2}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width =.5\textwidth]{images/rule-3.png}
% \caption{Fault detection sensitivity of rule 3}
% \label{fig: rule-3}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width =.5\textwidth]{images/rule-4.png}
% \caption{Fault detection sensitivity of rule 4}
% \label{fig: rule-4}
% \end{figure}
% {\color{red}JZ: Deng-please change all faults to faults for consistency including figures and texts}
\begin{figure}
\centering
\subfloat[Rule 1]{\includegraphics[width=.48\textwidth]{images/Adding_a_car.png}}\vfil

\subfloat[Rule 2]{\includegraphics[width=.48\textwidth]{images/Adding_a_bicycle.png}}\vfil

\subfloat[Rule 3]{\includegraphics[width=.48\textwidth]{images/Adding_a_pedestrian.png}}\vfil
\vspace{-5pt}

\subfloat[Rule 4]{\includegraphics[width=.48\textwidth]{images/Day2night.png}}\vfil

\subfloat[Rule 5]{\includegraphics[width=.48\textwidth]{images/Original2rainy.png}}\vfil
\caption{Fault detection sensitivity of rules}
\label{fig:rules}
\end{figure}

% \begin{figure}
% \centering
% \subfloat[Rule 1]{\includegraphics[width=.4\textwidth]{images/rule-1.png}}\hfil

% \subfloat[Rule 2]{\includegraphics[width=.4\textwidth]{images/rule-2.png}}\hfil

% \subfloat[Rule 3]{\includegraphics[width=.4\textwidth]{images/rule-3.png}}\hfil

% \subfloat[Rule 4]{\includegraphics[width=.4\textwidth]{images/rule-4.png}}\hfil

% \subfloat[Rule 5]{\includegraphics[width=.4\textwidth]{images/rule-5.png}}\hfil
% \caption{Fault detection sensitivity of rules}
% \label{fig:rules}
% \end{figure}

% \begin{figure}[ht]
% \centering
% \includegraphics[width=.5\textwidth]{images/rule-1.png}
% \includegraphics[width=.5\textwidth]{images/rule-2.png}
% \includegraphics[width=.5\textwidth]{images/rule-3.png}
% \includegraphics[width=.5\textwidth]{images/rule-4.png}
% \includegraphics[width =.5\textwidth]{images/rule-5.png}
% \caption{Fault detection sensitivity of rule 5}
% \label{fig: rule-5}
% \end{figure}
% \begin{figure*}

% \centering
% \subfloat[Fault detection sensitivity of rule 1]{\includegraphics[width=.3\textwidth]{images/rule-1.png}}\hfil
% \subfloat[Fault detection sensitivity of rule 2]{\includegraphics[width=.3\textwidth]{images/rule-2.png}}\hfil 
% \subfloat[Fault detection sensitivity of rule 3]{\includegraphics[width=.3\textwidth]{images/rule-2.png}} 

% \subfloat[Fault detection sensitivity of rule 4]{\includegraphics[width=.3\textwidth]{images/rule-4.png}}\hfil   
% \subfloat[Fault detection sensitivity of rule 5]{\includegraphics[width=.3\textwidth]{images/rule-5.png}}\hfil
% % \subfloat[F]{\includegraphics[width=3cm]{example-image-c}}
% \caption{Fault detection sensitivity of rules}\label{figure}
% \label{fig:rules}
% \end{figure*}


% We implemented proposed five metamorphic relations to generate corresponding follow-up test sets and then evaluate the fault coverage for five metamorphic relations on three autonomous driving models. Figure~\ref{} shows some generated test cases by different generaters in the metamorphic testing set generater toolkit.
% Table~\ref{tab:fault} shows the result of fault coverage of five generated metamorphic testing sets on three autonomous driving models. The results show that for every metamorphic testing set, the fault coverage is pretty high, which means all three autonomous driving models have robustness problems under the defined metamorphic testing scenarios. Those robustness problems cannot be observed if we only use normal metrics like MSE or MAE. 

% Comparing the three autonomous driving model, although they have similar MAE, their performances for those metamorphic tests are different. VGG16 model has lower fault coverage on the relations Day2night, original2rainy and add\_person; ResNet model has lower fault coverage on the relation add\_bicycle, and Epoch model has lower fault coverage on the relation add\_car. From the perspective of differential testing, we could use metamorphic testing to select the model which has the best performance in the specific scenario.  

% For each autonomous driving model, when we obtain the fault coverages for metamorphic relations, we would know in which kind of scenario the model does not perform well, which help us to add more training case about this scenario to re-train the autonomous driving model. However, {\color{red} explain we cannot do this now because we don't have the label for follow-up test set because our metamorphic relations are inequality relations.}

% \begin{table}[]
% \caption{Fault coverage}
% \label{tab:fault}
% \begin{tabular}{|l|l|l|l|}
% \hline
%               & Epoch & VGG16 & ResNet \\ \hline
% Day2night     &   100\%    &    95.2\%   &  98.0\%         \\ \hline
% Original2rain & 91.6\%      &   88.4\%    &     89.8\%      \\ \hline
% Add\_car      & 87.4\%      &   95.0\%    &     92.5\%      \\ \hline
% Add\_bicycle  & 78.5\%      &   83.9\%    &     78.5\%      \\ \hline
% Add\_person   & 100\%      &    62.5\%   &      77.3\%     \\ \hline
% \end{tabular}
% \end{table}

Figure \ref{fig:rules} shows the faults detected under five rules in different threshold settings. The x-axis denotes the deceleration range in MRs and y-axis denotes the faults that could be found given an expected deceleration range. To answering RQ1, we first look at the faults detected under default threshold setting for each rule.

For {\em Rule 1}, the deceleration threshold we set is 30\% to 40\%.
In this setting, we can detect $197$ faults on Epoch model. This implies that for Epoch model, $197$ out of $237$ prediction pairs violate the MR (i.e. $83.12\%$ fault coverage). 
ResNet with the same threshold has $207$ faults detected and fault coverage is $87.34\%$. VGG16 has $217$ faults detected and fault coverage is $91.56\%$ .
%Other two driving models VGG16 and ResNet in the same threshold have $217$ ($91.56\%$ fault coverage) and $207$ ($87.34\%$ fault coverage) faults detected for {\em Rule 1}.

For {\em Rule 2}, the deceleration threshold we set is 40\% to 50\%.
Overall the three models have similar number of faults, $146$ ($78.49\%$ fault coverage) for both Epoch and ResNet, and $156$ ($83.87\%$ fault coverage) for VGG16.
%and $146$ ($78.49\%$ fault coverage) for . 

For {\em Rule 3}, the deceleration threshold we set is 60\% to 70\%.
The numbers of faults detected for Epoch, VGG16 and ResNet are $299$ ($100\%$ fault coverage), $267$ ($89.30\%$ fault coverage), and $247$ ($82.61\%$ fault coverage), respectively. 

For {\em Rule 4}, the deceleration threshold we set is 0\% to 10\%.
The numbers of faults detected for Epoch, VGG16 and ResNet are $500$ ($100\%$ fault coverage), $476$ ($95.2\%$ fault coverage), and $490$ ($98\%$ fault coverage), respectively.

For {\em Rule 5}, the deceleration threshold we set is 10\% to 20\%.
The number of faults detected for Epoch, VGG16 and ResNet are  $458$ ($91.60\%$ fault coverage), $442$ ($88.40\%$ fault coverage), $449$ ($89.80\%$ fault coverage), respectively.

In summary, our results show that a large number of faults have been detected for all three driving models, with Epoch in total having $1600$ faults and $92.92\%$ fault coverage, VGG in total having $1558$ faults and $90.48\%$ fault coverage, ResNet in total having $1540$ faults and $89.43\%$ fault coverage.
The results show that with the rules we set and the corresponding thresholds, {\em RMT} is able to   uncover those faults judged by real-world traffic rules.

\begin{framed}
\noindent Result 1:  RMT could detect faults in driving models given threshold set by experts. 
\end{framed}
%Therefore, rule-based metamorphic testing could help detect robustness problems of autonomous driving models.
\subsection{RQ2: Fault Detection Sensitivity}
\vspace{-2pt}
\label{subsection:RQ2}
To answer RQ2, Figure~\ref{fig:rules} shows faults detected under five rules in different threshold settings.
For {\em Rule 1}, we observe a minimum fault coverage at $75.95\%$ and a maximal fault coverage at $100\%$. The difference between the minimum and maximum fault coverage (sensitivity range) is $24.05\%$. For VGG16 and ResNet, the sensitivity ranges are $14.35\%$ and $23.63\%$ respectively.

%the fault coverage change range is $16.88\%$ for Epoch with a minimum fault coverage at $83.12\%$ and a maximal fault coverage at $100\%$. For VGG16 and ResNet, the change ranges are $14.35\%$ and $23.63\%$ respectively.}
%{\color{blue} For {\em Rule 1}, the fault coverage change range is $16.88\%$ for Epoch with a minimum fault coverage at $83.12\%$ and a maximal fault coverage at $100\%$. For VGG16 and ResNet, the change ranges are $14.35\%$ and $23.63\%$ respectively.}
%with the lowest fault coverage of $83.12\%$ at the threshold of $30\%$ to $40\%$ and highest fault coverage of $100\%$ at the threshold of $90\%$ to $100\%$. The change rate is $14.35\%$ for VGG16 with the lowest fault coverage of $84.81\%$ at the threshold of $60\%$ to $70\%$ and highest fault coverage of $99.16\%$ at the threshold of $0\%$ to $10\%$. The change rate is $23.63\%$ for ResNet with the lowest fault coverage of $76.37\%$ at the threshold of $60\%$ to $70\%$ and highest fault coverage of $100\%$ at the threshold of $90\%$ to $100\%$.}
As observed from the {\em Rule 1} data, both VGG16 and ResNet have the lowest number of faults when the rule threshold (deceleration) is 60\% to 70\%. Since VGG16 and ResNet are more complex neural networks and also perform better in terms of Mean Absolute Error than Epoch, this observation may imply that the ground truth threshold for {\em Rule 1} shall be 60\% to 70\%. 
%\todo{TZ: what does the following sentence mean? Consider rewriting it with more clarity.}This may also be closely related to where the training sets for these two models are created (e.g., same country).

%Similarly to {\em Rule 1}, 
For {\em Rule 2}, the sensitivity range for Epoch, VGG16 and Resnet101 are $34.41\%$, $33.34\%$ and $21.51\%$ respectively.
We notice that Epoch has the lowest number of faults detected compared to the other two models at the deceleration threshold of 30\% to 40\% in {\em Rule 2}, which is $122$ ($65.59\%$ fault coverage), while VGG16 is consistent with Epoch to have the lowest number of faults detected in the same threshold, which is $124$ ($66.67\%$ fault coverage). For ResNet, it has the fewest faults detected at the threshold of 40\% to 50\%, which is 146 ($78.49\%$ fault coverage). Since the lowest thresholds for three models are very similar, which might imply the ground truth threshold for {\em Rule 2}, which shall be set 30\% to 50\%.

For {\em Rule 3}, the sensitivity range for Epoch, VGG16 and Resnet101 are $39.46\%$, $11.71\%$ and $27.76\%$ respectively. Epoch has the lowest number of faults detected at the threshold of 20\% to 30\%,  which is $181$ ($60.54\%$ fault coverage); while VGG16 and ResNet are consistent with the lowest number of faults detected at the threshold of 50\% to 60\%, which are $259$ ($86.62\%$ fault coverage) and $216$ ($72.24\%$ fault coverage) respectively. These results might imply the ground truth threshold for {\em Rule 3}, which shall be set 50\% to 60\%. 
%{\color{blue} Another possible reason for all three models perform bad is the ground truth threshold shall be set to 90\% to 100\%,
%where intuitively a vehicle shall fully stop if a person is in front of the vehicle.}
%according to our experience if a person is in front of our car, the speed should slow down to close 0.}

%For {\em Rule 4}, 
For {\em Rule 4}, the sensitivity range for Epoch, VGG16 and Resnet101 are $46.20\%$, $15\%$ and $25\%$ respectively. For {\em Rule 5}, the sensitivity range for Epoch, VGG16 and Resnet101 are $22.80\%$, $31.20\%$ and $21.6\%$ respectively. The fewest-faults thresholds for the three driving models vary. The lowest numbers of faults detected across models are all high with Epoch ($269$ and $53.8$\% fault coverage), VGG16 ($420$ and $84$\% fault coverage) and  ResNet ($375$ and $75$\% fault coverage).
Similarly for {\em Rule 5}, the lowest numbers of faults detected across three models are all high with Epoch ($386$ and $77.2$\% fault coverage), VGG16 ($344$ and $68.8$\% fault coverage) and ResNet ($392$ and $78.4$\% fault coverage). These results show that these driving models are most likely trained in day-time, non-rainy road images so that they have safety issues when time and weather change. 

In summary, we find different rule settings can affect fault detection with minimum sensitivity range $12.71$\% for VGG16 in {\em Rule 3} and maximum sensitivity range 46.2\% for Epoch in {\em Rule 4}.  This result shows that {\em Rule 3} can always capture faults in VGG16 irrespective of the threshold setting while {\em Rule 4} is quite sensitive of the threshold setting in capturing faults in Epoch.
%for capturing faults in Epoch, {\em Rule 4} requires domain expert knowledge in setting an appropriate threshold.

We also notice that {\em Rule 1} has the sensitivity range of $24.05\%$ where the minimum fault coverage by Epoch is $75.95\%$ and the maximum fault coverage by Resnet is $100\%$. The sensitivity range for {\em Rules 2-5} are $34.41\%$, $39.46\%$, $46.2\%$, and $31.2\%$ respectively. 
We have the conjecture that the lower the sensitive range for a rule, the more robust the rule will be to capture faults for driving models irrespective of the threshold settings.  For instance, in our study, {\em Rules 1, 2} and {\em 5} are more robust rules than others.

However, even after changing the threshold for each rule to its optimal value (leading to fewest faults), the numbers of total faults found for three models are $1138$ for Epoch (66.09\% fault coverage),  $1348$ for VGG (78.28\% fault coverage),  $1310$ for ResNet (76.07\% fault coverage), which are still very large. The finding also strengthens our answer to RQ1 where rule-based MRs can indeed detect faults. 

Moreover, based on these results, we can also know in which test scenarios driving models perform worst. This finding can lead us to add more training cases for those scenarios to help improve the training of autonomous driving models.  Another possible benefit is the conjecture that if we have more driving models under test, we can estimate the optimal threshold value for a particular rule by observing the threshold where majority of driving models have the fewest faults detected. 

\begin{framed}
\noindent Result 2:  RMT could test the overall performance of driving models in a specific scenario and find the optimal threshold where driving models . 
\end{framed}




% Figure \ref{fig:rules} shows the results of fault detection sensitivity for five metamorphic relations on the three autonomous driving models. 
% The x-axis denotes the threshold in metamorphic relations (i.e., deceleration range) and the y-axis denotes the suspicious faults that could be found given the certain threshold.

% Though we have defined the threshold for each rule, to investigate the driving models sensitivity for different thresholds (thus representing rules from different country/region), we plot the sensitivity graph that sets $10$ deceleration thresholds from (0, 0.1) to (0.9, 1) for each rule (i.e., from no deceleration to full stop with 10\% deceleration as the range).

% {\color{red}JZ-Deng, I have changed the section quite heavily and for those missing stats, I have given you the comments.  I said fault number, but please give also the fault percentage along with the number.}
% For {\em Rule 1},the deceleration threshold we originally set is 30\% to 40\%.
% In this setting, we can detect $197$ faults on Epoch model.This implies for Epoch model, $197$ out of $237$ prediction pairs violate the metamorphic relation (i.e. $83.12\%$ fault coverage). Other two driving models in the same threshold have $217$ and $219$ violations detected ({\color{red}JZ: Deng-give the number of faults detected for these two models for this threshold} for {\em Rule 1}. {\color{red}JZ: Deng, I added the below analysis, please check whether it is correct especially the claims}One interesting observation from the {\em Rule 1} data is both VGG16 and ResNet have the lowest number of violations when the deceleration threshold is 60\% to 70\%.  Since VGG16 and ResNet are more complex neural networks and better performing driving models (in terms of Mean Absolute Error) than Epoch, it might point out the ground truth threshold for {\em Rule 1} shall be 60\% to 70\%. This might also be closely related to where the training sets for these two models are created (e.g., same country).

% For {\em Rule 2}, Overall the three models have similar number of faults in the range from $145$ to $160$.
% We also notice that Epoch has the lowest number of metamorphic relation violations at the deceleration threshold of 30\% to 40\% {\color{blue}, which is $122$}, while VGG16 is consistent with Epoch to have the lowest number of violations in the same threshold {\color{blue}, which is $124$}. ResNet has the fewest violdations at the threshold of 40\% to 50\% {\color{blue}, which is 146}. These results might point out the ground truth threshold for {\em Rule 2}, which shall be set 30\% to 50\%.

% For {\em Rule 3}, the numbers of faults for Epoch, VGG16 and ResNet are $299$ ({\color{blue}$100\%$}), $267$ ($89.30\%$), and $247$ ($82.61\%$) respectively. Epoch has the lowest number of violations at the threshold of 20\% to 30\% {\color{blue}, which is $181$ ($60.54\%$)}; while VGG16 and ResNet10 are consistent with the lowest number of violations at the threshold of 50\% to 60\%{\color{blue}which are $259$ ($86.62\%$) and $267$ ($89.30\%$) respectively}. These results might point out the ground truth threshold for {\em Rule 3}, which shall be set 50\% to 60\%. {\color{red} YD: I think for rule 3, all three models perform bad because according to our experience if a person is in front of our car, the speed should slow down to close 0.}

% For {\em Rule 4}, the numbers of faults for Epoch, VGG16 and ResNets are similar ($500$, $476$, and $490$, respectively). However, the fewest-violation thresholds for the three driving models vary. The lowest numbers of violations across three models are all very high with Epoch ($269$ and $53.8$\%), VGG16 ($420$ and $84$\%) and  ResNet ($375$ and $75$\%){\color{red}JZ: Deng-give the fault number here}.  Similarly for {\em Rule 5}, the number of faults for Epoch, VGG16 and ResNet are close ($458$, $442$, $449$, respectively).  The lowest number of violations across three models are all very high with Epoch ($386$ and $77.2$\%), VGG16 ($390$ and $78$\%) and  ResNet ($392$ and $78.4$\%){\color{red}JZ: Deng-give the fault number here}.  These results show that these driving models are most likely trained in day-time, non-rainy road images so that they have robustness issues when time and weather change. 



%Depending on the rules we set, for every metamorphic test set, the fault coverage on three driving models are pretty high (more than 60\%), which shows those driving models have robustness problems under defined metamorphic testing scenarios. Those robustness problems cannot be observed if we only use normal metrics like MSE or MAE.

%For {\Rule 4} and {\em Rule 5}, the number of detected faults on three models are close. Depending on the rules we set, for every metamorphic test set, the fault coverage on three driving models are pretty high (more than 60\%), which shows those driving models have robustness problems under defined metamorphic testing scenarios. Those robustness problems cannot be observed if we only use normal metrics like MSE or MAE.
%For {\em Rule 3}, the number detected faults for Epoch, VGG16 and ResNet are 300, 263, and 243 respectively. For rule 4 and rule 5, the number of detected faults on three models are close. Depending on the rules we set, for every metamorphic test set, the fault coverage on three driving models are pretty high (more than 60\%), which shows those driving models have robustness problems under defined metamorphic testing scenarios. Those robustness problems cannot be observed if we only use normal metrics like MSE or MAE.




% {\color{red}JZ: Miryung/Tianyi, I have made some claims here and please check whether they are too big}
% In summary, we notice a  large number of faults (Epoch $1599$, i.e., $92.86\%$ fault coverage; VGG $1558$, i.e., $90.48\%$ fault coverage; ResNet $1551$, i.e., $90.10\%$ fault coverage) from our results.  Even after changing the threshold for each rule to its optimal value (leading to fewest violations), the number of total faults found (Epoch $xxMIN$, VGG $xxMIn$, ResNet $xxxMIn$) {\color{red}JZ: Deng-give the fault number here for each driving models} is still very large.
% Also based on the rules we set and the corresponding metamorphic relations, we could detect faults of autonomous driving models on different test scenarios while those faults cannot be revealed by normal metrics like MSE and MAE. Therefore, rule-based metamorphic testing could help detect robustness problems of autonomous driving models. In addition, based on the test results, we could know in which test scenarios models perform worst. Then we could add more training cases of those scenarios to help improve the training of autonomous driving models.  Moreover, if we have more driving models under test, we can estimate the optimal threshold value for a particular rule by observing the threshold where majority of driving models have the fewest faults detected. 
%In summary, based on the rules we set and the corresponding metamorphic relations, we could detect faults of autonomous driving models on different test scenarios while those faults cannot be revealed by normal metrics. Therefore, rule-based metamorphic testing could help detect robustness problems of autonomous driving model. In addition, based on the test result, we could know in which test scenarios models perform worst. Then we could add more training cases of those scenarios to help improve the training of autonomous driving models.  

% \subsection{Manual Evaluation}
% {\color{red} I analyze all result together and do not discuss the image realistic level.}
% Tables \ref{tab:kappa_1}-\ref{tab:kappa_5} show the results of manual evaluation for the realistic level of generated metamorphic images and reasonable level of predicted speed changes (i.e., deceleration). 
% For each table, the first two rows demonstrate the mean value of image realistic level and model prediction change reasonable level. The last row shows the weighted kappa score for each metric. The kappa score shows the agreement of two raters.  The kappa score equaling to $1$ means two raters have the totally same rating while $-1$ means the opposite situation. For all rules, most model prediction change reasonable level values are smaller than $3$ and some of them are even smaller than $2$. Meanwhile most kappa scores are larger than 0 and some of them achieve 0.4-0.6, which means the evaluation of two raters are highly in agreement.  From the result, we can know that both two raters think the speed changes predicted by the three driving models are not reasonable (thus revealing faults). These findings are consistent with our quantitative analysis for the fault detection. 

% Another interesting observation is the image realistic level overall is not high. It mainly lies in the transformation engine we used for {\em Rules 1-3}. As the added object is created by a GAN neural network and we do not have enough dataset to train this specific GAN. The added object does not have enough features to make the object real enough though vehicle, pedestrian and bicycle are close to real as shown in Fig.~\protect\ref{fig:pix2pix_generate}\subref{fig:generate_f}, \ref{fig:pix2pix_generate}\subref{fig:generate_g}, and \ref{fig:pix2pix_generate}\subref{fig:generate_h}, respectively.
% {\color{red}JZ: Deng-give sub-figure labels for adding a car, adding a pedestrian and adding a bicycle}.  

%five rules. For each table, the first two rows demonstrate the mean value of image realistic level and model prediction change rationality level. The last row shows the weighted kappa score for each metric. The kappa score shows the agreement of two raters.  The kappa score equaling to $1$ means two raters have the totally same rating while $-1$ means the opposite situation. For all rules, most model prediction change rationality level values are smaller than 3 and some of them are even smaller than 2. Meanwhile most kappa scores are larger than 0 and some of them achieve 0.4-0.6, which means the evaluation of two raters are highly in agreement.  From the result, we can know that both two raters think driving models cannot produce the reasonable predictions under test scenarios defined by metamorphic relations. 

\begin{table}[]
\caption{Evaluation of rule 1{\color{red}The title may need to change}}
\label{tab:kappa_1}
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{}                                     & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}(Mean of) image \\ realistic level\end{tabular}} & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}(Mean of) model prediction change\\ rationality level\end{tabular}} \\ \cline{3-5} 
                                                      &                                                                                             & Epoch                               & VGG16                               & ResNet                              \\ \hline
rater1                                                & 3.224                                                                                        & 2.667                                & 3.286                                & 3.034                                   \\ \hline
rater2                                                & 3.646                                                                                        & 2.816                               & 3.490                                & 3.088                                   \\ \hline
\begin{tabular}[c]{@{}l@{}}Kappa\\ score\end{tabular} & -0.057                                                                                      & 0.567                               & 0.596                               & 0.555                                  \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\caption{Evaluation of rule 2{\color{red}The title may need to change}}
\label{tab:kappa_2}
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{}                                     & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}(Mean of) image \\ realistic level\end{tabular}} & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}(Mean of) model prediction change\\ rationality level\end{tabular}} \\ \cline{3-5} 
                                                      &                                                                                             & Epoch                               & VGG16                               & ResNet                              \\ \hline
rater1                                                & 3.881                                                                                        & 1.5                                & 1.556                                & 1.595                                   \\ \hline
rater2                                                & 4.960                                                                                        & 1.325                                & 1.317                                & 1.548                                   \\ \hline
\begin{tabular}[c]{@{}l@{}}Kappa\\ score\end{tabular} & 0.029                                                                                      & -0.092                               & 00593                               & 0.111                                  \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\caption{Evaluation of rule 3{\color{red}The title may need to change}}
\label{tab:kappa_3}
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{}                                     & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}(Mean of) image \\ realistic level\end{tabular}} & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}(Mean of) model prediction change\\ rationality level\end{tabular}} \\ \cline{3-5} 
                                                      &                                                                                             & Epoch                               & VGG16                               & ResNet                              \\ \hline
rater1                                                & 3.220                                                                                        & 1.387                                & 2.310                                & 2.399                                   \\ \hline
rater2                                                & 5.095                                                                                        & 2.048                                & 3.214                                & 2.792                                   \\ \hline
\begin{tabular}[c]{@{}l@{}}Kappa\\ score\end{tabular} & 0.006                                                                                      & 0.065                               & 0.299                               & 0.407                                  \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\caption{Evaluation of rule 4{\color{red}The title may need to change}}
\label{tab:kappa_4}
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{}                                     & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}(Mean of) image \\ realistic level\end{tabular}} & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}(Mean of) model prediction change\\ rationality level\end{tabular}} \\ \cline{3-5} 
                                                      &                                                                                             & Epoch                               & VGG16                               & ResNet                              \\ \hline
rater1                                                & 3.336                                                                                        & 1.963                                & 1.792                                & 1.982                                   \\ \hline
rater2                                                & 3.866                                                                                        & 2.668                                & 2.447                                & 2.461                                   \\ \hline
\begin{tabular}[c]{@{}l@{}}Kappa\\ score\end{tabular} & -0.0715                                                                                      & 0.279                               & 0.274                               & 0.453                                  \\ \hline
\end{tabular}
\end{table}

\begin{table}[]
\caption{Evaluation of rule 5{\color{red}The title may need to change}}
\label{tab:kappa_5}
\begin{tabular}{|l|l|l|l|l|}
\hline
\multirow{2}{*}{}                                     & \multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}(Mean of) image \\ realistic level\end{tabular}} & \multicolumn{3}{l|}{\begin{tabular}[c]{@{}l@{}}(Mean of) model prediction change\\ rationality level\end{tabular}} \\ \cline{3-5} 
                                                      &                                                                                             & Epoch                               & VGG16                               & ResNet                              \\ \hline
rater1                                                & 3.304                                                                                        & 2.270                                & 2.214                                & 2.450                                   \\ \hline
rater2                                                & 4.461                                                                                        & 2.731                                & 2.538                                & 2.641                                   \\ \hline
\begin{tabular}[c]{@{}l@{}}Kappa\\ score\end{tabular} & 0.015                                                                                      & 0.427                               & 0.449                               & 0.461                                  \\ \hline
\end{tabular}
\end{table}

% 


% \begin{figure*}[!t]
% \begin{minipage}[c]{\linewidth}
%   \begin{subfigure}[b]{0.32\linewidth}
%     \includegraphics[width=\linewidth]{images/evaluation-epoch.png}
%     \caption{Epoch model}
%     \label{fig:distance}
%   \end{subfigure}
%   %
%   \begin{subfigure}[b]{0.32\linewidth}
%     \includegraphics[width=\linewidth]{figures/example-hexToString.png}
%     \caption{VGG16 model}
%     \label{fig:hexstring}
%   \end{subfigure} 
%   %
%   \begin{subfigure}[b]{0.32\linewidth}
%     \includegraphics[width=\linewidth]{figures/example-android.png}
%     \caption{ResNet model}
%     \label{fig:android}
%   \end{subfigure}
%   \end{minipage}
%   \caption{{\tool} code template examples}
%   \label{fig:examples}
% \end{figure*}

\begin{figure*}[!t]
\begin{minipage}[c]{\linewidth}
  \subfloat[]{\includegraphics[width=.33\textwidth]{images/evaluation-epoch.png}\label{fig:eva-epoch}}\hfil
\subfloat[]{\includegraphics[width=.33\textwidth]{images/evaluation-vgg16.png}\label{fig:eva-vgg16}}\hfil 
\subfloat[]{\includegraphics[width=.33\textwidth]{images/evaluation-resnet101.png}\label{fig:eva-ResNet}}\hfil 
  \end{minipage}
  \caption{Human Assessment of Speed Prediction Change Made by Three Driving Models in a 7-Point Likert Scale}
  \label{fig:human}
\end{figure*}

\subsection{RQ3: Qualitative Analysis}
\label{subsection:RQ3}
{\color{blue} In human evaluation, six participants with driving experiences rates for what extend the speed prediction changes looks reasonable in a 7-point likert scale, from extremely unreasonable (0 point) to extremely reasonable (7 points), and scores are shown in the Figure \ref{fig:human}}.
%Figure \ref{fig:human} shows the scores given by human raters about to what extent the speed prediction looks reasonable to them in a 7-point likert scale. 
For Epoch model, rater $1$ rates most test case pairs in the range [1, 3], which means the rater thinks most predictions are not reasonable and some of predictions are most unreasonable. For raters $2$, $3$, $5$, and  $6$, their ratings are mostly in the unreasonable prediction range [2, 4]. Only rater $4$ provides higher ratings and it seems that rater $4$ always rates higher than other raters across three models, which implies rater $4$ may have different experience of judging the reasonable level than others. The mean of ratings across all raters for Epoch model is $2.673$, which is a low prediction reasonable level and suggests that raters think the predictions of Epoch models on generated metamorphic road images are incorrect.  For each rule, we calculated the mean ratings of six raters, which are $2.950$, $2.201$, $2.397$, $3.035$, and $2.611$ respectively for {\em Rules 1-5}. This shows raters think predictions of Epoch model on the metamorphic road images generated from our rules are largely incorrect, which is consistent with our findings in RQ1 and RQ2.

The results of VGG16 and ResNet are a little better than those of Epoch but their predictions are also in the low reasonable range. For VGG16, most ratings of raters $1$, $2$, $3$, $5$ and $6$ are in the range [1, 4]. The mean rating of VGG16 model's prediction is $2.711$ across metamorphic road images generated from our five rules and the individual mean ratings for
VGG16 model's prediction across road images generated from 
{\em Rules 1-5} are $3.093$, $2.122$, $2.812$, $2.829$, and $2.596$ respectively. For ResNet, the mean ratings of six raters for its prediction across road images generated from 
{\em Rules 1-5} are $3.170$, $2.286$, $2.913$, $3.023$, $2.748$ respectively and the mean rating on ResNet model is $2.852$. All values are in the range [2, 4). Such a result implies that  
raters consider predictions of VGG16 and ResNet on road images generated from our rules as largely incorrect, which is also consistent with our findings in RQ1 and RQ2.


In summary, from our user study, raters think all three driving models have very poor performance in predicting speed based on the metamorphic road images generated from our proposed {\em RMT} tool. The result shows the faults detected by RMT are truthful with a fairly high confidence level of $2.745$ mean rating across all the driving models (i.e., mean rating of $2.673$ for Epoch, $2.711$ for VGG16  and $2.852$ for ResNet).

\begin{framed}
\noindent Result 3: The testing results of RMT are truthful according to human validation. 
\end{framed}
%To sum up, from the manual evaluation, raters think all three models have low prediction correctness level for five test scenarios generated by RMT, which is consistent with the experiment RQ1 that many faults of three models are detected by RMT. Therefore, the manual evaluation proves that RMT can actually detect faults of autonomous driving models. }
% \begin{table}[]
% \caption{Mutation score}
% \label{tab:fault}
% \begin{tabular}{|l|l|l|l|}
% \hline
%               & Epoch & VGG16 & ResNet \\ \hline
% Source test set     &       &    0.0112   &          \\ \hline              
% Day2night     &      &    0.0051   &          \\ \hline
% Original2rain &      &   0.0062  &           \\ \hline
% Add\_car      &       &   0.4545    &          \\ \hline
% Add\_bicycle  &      &   0.0229    &          \\ \hline
% Add\_person   &      &    0.0167  &         \\ \hline
% \end{tabular}
% \end{table}



\subsection{Threats to validity}
For the image generation methods, we used UNIT and Pix2PixHD. These two GAN models were used to generate real scenes based on semantic labels. By changing objects in semantic labels, our model could make changes on the real driving scenes. However, restricted by the performance of these two GAN models, the generated images are not realistic enough.  With more datasets to train these two GANS or with a much powerful GAN, we can replace the current ones in our {\em RMT} to achieve better results. 

Moreover, Pix2PixHD model we used for {\em Rules 1-3} cannot directly make changes of items on the original image, and it could only add, move, or delete existing items (one of the instances in the semantic label maps) based on semantic label maps without the capabilities of adding new items. This restriction can also be removed by finding a more powerful alternative for the transformation engine.
%from segmentation generated images, without changes on other items. These two problems would be solved in future study by improving or changing these models. 
We chose cityscapes as our dataset mainly due to the dataset has built-in semantic label map for each road image. A highly accurate semantic label map is essential for Pix2PixHD model we used for {\em Rules 1-3} to generate a truthful road image. For the Udacity dataset, although it is wildly used for autonomous driving, semantic labels of this dataset are not provided and existing semantic segmentation utilities can not create semantic labels on the dataset with the quality we wanted, thus we could not use the Udacity dataset in our paper to implement {\em Rules 1-3}. This limitation can be removed by finding an improved semantic segmentation tool.
%As the pix2pixHD model is trained on the cityscapes dataset, to improve the reality of generating dataset, we use cityscapes in experiments. For the Udacity dataset, although it is wildly used for autonomous driving, semantic labels of this dataset are not provided and existing semantic segmentation utilities can not provide the realistic effects we wanted,  thus we could not use this dataset in this paper to implement {\em Rules 1-3}.
In our work, a fault is said to be detected when an MR is violated. 
However, in the context of autonomous driving, the violation of an MR only implies the potential of erroneous behaviour, that is, the detected fault is a ``suspicious'' one.  We used the qualitative user study to mitigate this validity issue and our results show the violation of an MR is a fault with very high probability.
%
%
%In the rest of the paper, we use ``suspicious faults'' and ``metamorphic relation violations'' (or briefly ``violations'') interchangeably.  
%For the autonomous driving task we used in our framework, compared with the steering angle prediction task, more relations could be defined on the speed prediction task. Also, as there already exists some evaluation tools based on the steering angle prediction task, our method could also be considered as a supplement method of existing methods.
%However, to solve the speed prediction task, recurrent models would perform better than  convolutional models. While limited by the discontinuous images in the cityscapes dataset which is required by recurrent models, we have to choose the three CNN models. 

% {\color{red}JZ: Deng, please check this statement is correct}
%Epoch, VGG16 and ResNet. Epoch is a good model on the Udacity dataset, and always used as the baseline for the steering angle prediction task. For VGG16 and ResNet model, they perform well on computer vision task, and are wildly used in the models of autonomous car systems.




% In this paper, we did not compare our framework with other similar MT based approaches (e.g.,  {\em DeepRoad} and {\em DeepTest}) with reasons. Firstly, we used the speed prediction labels to evaluate the effect of our approach, rather than the steering angle prediction labels in these two models. In addition, we used rule-based MR which includes both equality relation (no changes for the output from metamorphic test set) and inequality relation (with changes for the output from metamorphic test set). Our approach is considered as the superset, and thus we have integrated the GAN used by {\em DeepRoad} for {\em Rule 4} and OpenCV used by {\em DeepTest} for {\em Rule 5}.


{\color{blue} Comparing with {\em DeepTest} and {\em DeepRoad}, our main focus is to design and evaluate inequality metamorphic relations, while {\em DeepTest} and {\em DeepRoad} only support equality relations. Therefore, it is not really a head-to-head comparison. Yet we want to clarify that the declarative language in RMT is capable of expressing those equality relations in {\em DeepTest} and {\em DeepRoad}. RMT also implements the affine transformations in {\em DeepTest} and the GAN-based transformations in {\em DeepRoad}. Therefore, RMT is a more general framework compared with previous work.}


%the evaluation method in our framework is mutation score, rather than the neural coverage in DeepRoad and DeepTest. While comparing with the mutation method proposed by DeepMutation, 4 out of 8 mutation strategies we used in our framework, because weight shuffling, layer deactivation, layer addition and Act. Fun. Remov. methods would change the structure of our test models, which obey the requirements of mutation testing. Furthermore, in this paper, the speed variation threshold is setted according to daily experience, while in the real application, the reasonable threshold should be set by experts. 


